Harmonics of Learning: Universal Fourier Features Emerge in Invariant Networks

In this work, we formally prove that, under certain conditions, if a neural network is invariant to a finite group then its weights recover the Fourier transform on that group. This provides a mathematical explanation for the emergence of Fourier features -- a ubiquitous phenomenon in both biological and artificial learning systems. The results hold even for non-commutative groups, in which case the Fourier transform encodes all the irreducible unitary group representations. Our findings have consequences for the problem of symmetry discovery. Specifically, we demonstrate that the algebraic structure of an unknown group can be recovered from the weights of a network that is at least approximately invariant within certain bounds. Overall, this work contributes to a foundation for an algebraic learning theory of invariant neural network representations.

==> scrach.tex <==
% A notable and to-date unexplained phenomenon within deep learning theory is that of 

% The phenomenon of \textit{convergent learning} \cite{li2015convergent} is a notable property of deep learning. 

% \textit{Convergent learning} \cite{li2015convergent} or \textit{universality} \cite{olah2020overview}



% prev:
%Artificial neural networks trained on natural data exhibit a striking phenomenon: regardless of exact initialization, dataset, or training objective, models trained on the same data domain frequently converge to similar learned representations \cite{li2015convergent}. For example, the early layer weights of diverse image models tend to converge to Gabor filters and color-contrast detectors \cite{olah2020overview}. Remarkably, many of these same features are observed in the visual cortex \cite{hubel1959receptive, hass2013v1, willeke2023deep}, suggesting a form of \textit{representational universality} that transcends biological and artificial substrate. While such findings are empirically well-established in the \textit{mechanistic interpretability} literature \cite{rauker2023toward}, the field still lacks theoretical explanation.

% A suite of results in the field of \textit{mechanistic interpretability} \cite{rauker2023toward} aims to reverse-engineer the weights of trained machine learning models. A suite of results in this direction has uncovered regularities for emergent features in artificial neural networks \cite{conmy2023towards}. Although these phenomena are empirically well-established, the field still lacks theoretical explanation.




% Our work compliments the equivariant convolutional neural network literature \cite{cohenc16, pmlr-v80-kondor18a} since our models can be used to form an efferent invariant layer for downstream processing \cite{sanborn2023bispectral, sanborn2024general}.

% prev: 
%This work represents a significant attempt to provide theoretical grounding for the phenomenon of convergent learning (i.e. the \textit{universality hypothesis} \cite{olah2020overview, moschella2022relative}). A suite of earlier theoretical works \cite{isely2010deciphering, hillar2015can, garfinkle2019uniqueness} tackled a related problem, establishing guarantees that a model will recover (up to scaling) the true underlying basis of data generated as a sparse linear combination of those bases. Our findings here suggest [...] Given the centrality of invariance to many machine learning tasks, our proof is able to explain a broad class of convergent learning phenomena, in a broad class of neural network architectures, while providing a new perspective on classical neuroscience results. As such, it sets a foundation for a learning theory of representations in artificial and biological neural systems, grounded in the mathematics of symmetry.

 % any network that accurately encodes sparse linear combinations of a given set of basis functions recovers those bases up to scaling \cite{hillar2015can, garfinkle2019uniqueness}, a finding leveraged for an unsupervised communication model between brain regions \cite{isely2010deciphering}. More generally,

 % it sets a foundation for future work in mechanistic interpretability, opening the door for further mathematical explanation of the emergence of universal features in artificial and biological learning systems. 
 
 
 % In particular, we focus on the emergence of \textit{Fourier features} in artificial neural networks, and are able to derive a theoretical guarantee for the emergence of these features in models trained on tasks that require \textit{invariance} or \textit{equivariance} to the actions of a \textit{group of transformations} (e.g. planar translation or rotation). 




% The standard Fourier transform is a special case of more general Fourier transforms on groups \cite{rudin1964fourier}, which can be defined by replacing the standard Fourier basis\textemdash equivalent to the irreducible representations of the group of cyclic translations\textemdash with the irreps of other compact groups. For example, Fourier transforms can be defined on the groups of 2D and 3D rotation using the bases of disk harmonics or spherical harmonics. Notably, these more general Fourier features have been observed to emerge in neural networks trained on tasks that require invariance or equivariance to different groups \cite{sanborn2023bispectral, fiquet2023polar}, and have been suggested as an explanation for features observed throughout the mammalian visual cortex \cite{}. 

% \footnote{Mathematically, the Fourier transform is a projection of a signal onto the \textit{irreducible representations} of a group\textemdash cyclic translation in the standard case. This gives it the property of \textit{equivariance} to the group. Fourier transforms can be defined on other groups by replacing the standard Fourier basis with other irreducible group representations. For example, the disk harmonics or spherical harmonics can be used to define Fourier transforms on the groups $SO(2)$ and $SO(3)$ or 2D and 3D rotations.} 

% In this paper, we explain the emergence of both localized and general group-Fourier features in neural networks.

% In this paper, we suggest that these empirical observations may be explained by the ubiquity of \textit{invariance} and \textit{equivariance} in the structure of many tasks relevant for perception and intelligence. Our proof [...]. Concretely, our contributions are as follows:

% \begin{itemize}
%     \item We prove that if a neural network of a certain kind is invariant to a group $G$, then its weights must (almost) coincide with the irreducible unitary representations of that group.
%     \item Our proof covers both commutative and non-commutative groups, and a general class of neural network architectures, including convolutional networks and multi-layer perceptrons with [...] activation functions, including [...] and polynomial activations. 
%     \item We demonstrate this convergent learning in a suite of empirical experiments, and show that across initializations, on a diverse set of datasets and network architectures, models consistently converge to the theoretically predicted representations.
% \end{itemize}


%We provide a one-page introduction to these mathematical foundations in Appendix \ref{appendix:math}.



% We start by recalling the notion of a group. Intuitively, a group is an algebraic object whose elements represent abstract symmetries. The latter can be composed and inverted, leading to the following definition.  


% In this section we outline the principles of group theory together with harmonic analysis over groups. For a complete treatment we refer to \cite{folland2016course}. 



% We first review harmonic analysis of signals over groups. 


% Moreover, for the following sections we assume that $G$ is commutative, which greatly simplifies harmonic analysis. We discuss the non-commutative case in Section \ref{sec:nonabelian}. 


% \begin{remark}\label{rem:gract}
% \end{remark}


% On the same note, Spectral Networks for non-commutative groups can be defined as follows. Given a matrix $W \in \mathbb{C}^{d \times d}$, $d = |G|$, we think of it as a concatenation of $k$ tensors $W_i \in \mathbb{C}^{ d_i \times d_i \times d}$, where $d_1, \cdots, d_k$ are the dimensions of all the irreducible unitary representations of $G$. Given a multi-index $\underline{i} = (i_1, \cdots, i_n)$, we denote $d_{\underline{i}} = d_{i_1} \cdots d_{i_n}$. The \emph{Spectral Network} is then defined as the collection of parametric maps $\varphi_{\underline{i}}(W, \cdot):  \ \free{G} \simeq \mathbb{C}^d \rightarrow \mathbb{C}^{d_{\underline{i}} \times d_{\underline{i}}}$ given by: 
% \begin{equation}\label{eq:ncspecnet}
% \varphi_{\underline{i}}(W, x) =  ( W_{i_1} x )  \otimes \cdots \otimes (W_{i_n} x) \  \left( W_{i_1}^{\dagger} \overline{x} \ \otimes   \cdots \otimes W_{i_n}^{\dagger} \overline{x} \right).
% \end{equation}



% We first focus on the commutative case, implying that $V = \mathbb{C}$ and therefore $W \in \free{G}$. Two examples of unitarily injective maps are: 
% \begin{itemize}
% \item \textit{Spectral Networks}: the model discussed in Section \ref{sec:specnet} obtained for a constant multi-index i.e.,
% \begin{equation}
% \varphi(W, x) = (Wx)^n \ \overline{W^{\odot n}x}
% \end{equation}
% for some $n > 0$. 
% \item \textit{McCulloch-Pitts Neurons}: a model of the form 
% \begin{equation}
%  \varphi(W,x) = \sigma(W x ),
% \end{equation}
% where $\sigma: \ \mathbb{C} \rightarrow \mathbb{C}$ is a map playing the role of an activation function. For $\sigma(z) = |z|^2$, this model reduces to a Spectral Network with $n=1$.    
% \end{itemize}

% Both the class of models above can be seen to satisfy the condition of unitarily injectivity, albeit with an assumption on $\sigma$.


% We now focus on another model common in neuroscience and machine learning, which we refer to as (complex) \emph{McCulloch-Pitts networks}. 



% Next, we discuss the case of classical deep networks. We model the latter as $\varphi(W, x) = \chi(|W(x)|^2)$, where $W \in \mathcal{W} = \free{G} \otimes \mathbb{C}^k$ and $|\cdot|$ denotes the component-wise absolute value. Here, $k$ is the number of neurons in the first hidden layer of the network, while $\chi \colon \mathbb{R}_{\geq 0}^k \rightarrow \mathbb{R}$ is the head of the network, encompassing all the layers after the first one. Note that since typical neural networks are real-valued, we combine real and complex models. Namely, the first layer of $\varphi$ is complex, and its output is fed into the real head $\chi$ by taking squared absolute values. 

% % In what follows, we say that $\varphi(W,x)$ \emph{generically} has unitary hidden symmetries if Definition \ref{def:symm} holds for almost all $W \in \mathcal{W}$ i.e., if it holds in an open dense subspace of $\mathcal{W}$ (with the usual Euclidean topology). 
% Differently from Section \ref{sec:theoretical-results}, for the next result we will restrict $\mathcal{W}$ to the subspace of $\free{G} \otimes \mathbb{C}^k$ consisting of $W$ such that the components $W_i$ are orthonormal. This implies, in particular, the constraint $k \leq |G|$. Note that $\mathcal{W}$ is closed by the actions of $G$ and $\textnormal{U}(\mathbb{C})$. The orthonormality condition is anyway necessary in order to recover the Fourier transform, as stated in Corollary \ref{mainpropnc}.  

% \begin{proposition}\label{prop:deepnets}
% Suppose that there is an open subspace $O \subseteq \mathbb{R}_{\geq 0}^k$ containing $0$ where $\chi$ is affine with distinct non-vanishing coefficients i.e., $\chi(z) = \sum_i a_i z_i + b$ for $z \in O$ with $0 \not = a_i \not = a_j$ for $i \not = j$. Then $\varphi(W, x) = \chi(|W(x)|^2)$ has unitary symmetries. 
% \end{proposition}  
% We refer to the Appendix for a proof. Since typical (real-valued) deep neural networks have piece-wise linear activations functions such as (leaky) ReLU, they define piece-wise affine maps and therefore satisfy the hypothesis from Proposition \ref{prop:deepnets}. Moreover, the hypothesis on the coefficients $a_i$  is \emph{generic} i.e., it defines an open dense subset of $(a_1, \cdots, a_k) \in \mathbb{R}^k$. 



% \begin{lemm}\label{polarlemm}
% Let $n \geq d$ and $A,B \in \mathbb C^{n \times d}$. If $AA^{\dagger} = BB^{\dagger}$ then $A = BW$, in which $W = V^{\dagger}U$ for some $U,V \in \mathbb C^{n \times d}$ with orthonormal rows.
% \end{lemm}

% \begin{proof}
% From the polar decomposition for matrices (see \cite[Theorem 3.1.9]{horn1994topics}), we know that:
% \begin{equation} 
% A = PU, \ B = Q V,
% \end{equation}
% where $P,Q$ are Hermitian positive semidefinite and $U,V$ have orthonormal rows.  Also, $P^2 = AA^{\dagger} = BB^{\dagger} = Q^2$ from which it follows that $P = Q$ by uniqueness of square roots of positive semidefinite Hermitian matrices (see \cite[Theorem 7.2.6]{horn2012matrix}).  In particular, we have:
% \begin{equation}
% A = PU = QU = Q(VV^{\dagger})U = 
% QV(V^{\dagger}U) = BW,
% \end{equation}
% with $W$ as in the statement of the lemma.
% \end{proof}

%We remark that if $n < d$, the matrix $W$ above is necessarily singular, which follows from the fact that the rank of a product of matrices is at most the rank of each. 



% \subsection{Proof of Proposition \ref{mainrelax}}

% In order to prove the Proposition, we will need the following technical fact from linear algebra. 


% \begin{lemm}\label{lemmrelax}
% Let $H$ be a finite-dimensional complex Hilbert space, $v,w \in H$ normal  and $\varepsilon \in \mathbb{R}_{> 0}$. Suppose that for every normal $x$ orthogonal to $w$, it holds that $| \ \langle x, v\rangle \ | < \varepsilon$. Then there exists $\rho \in \textrm{U}(1)$ such that 
% \begin{equation}
% \| v - \rho w \| < \sqrt{2\left( 1- \sqrt{1 -   \varepsilon^2 } \right) }. 
% \end{equation}
% \end{lemm}

% \begin{proof}
% Consider an orthogonal decomposition $v = \langle w_1, v \rangle  w_1 + \langle w_2,  v \rangle w_2$, where $w_1 \in w^\perp$ is normal and $w_2 = \rho w$ for some $\rho \in \textnormal{U}(1)$ such that $\langle w_2, v \rangle \in \mathbb{R}_{\geq 0}$. It follows that
% % \begin{equation}
% % |\ \langle \widetilde{w}, x \rangle \ | = | \  \langle w, x \rangle   - \langle  w -  \widetilde{w}, x \rangle\ | \leq \varepsilon + \| \widetilde{w} - w \| = \varepsilon + \sqrt{2}. 
% % \end{equation}
% \begin{equation}
% 1 = \| v \|^2 = | \ \langle w_1, v \rangle\ |^2 +    \langle w_2, v \rangle ^2.
% \end{equation}
% The hypothesis implies then that $  \ \langle w_2, v \rangle\   > \sqrt{1 -   \varepsilon^2 } $. Therefore, 
% \begin{equation}
% \| v - w_2 \|^2 = 2 - 2\langle w_2, v \rangle  <    2\left( 1- \sqrt{1 -   \varepsilon^2 } \right) 
% \end{equation}
% as desired. 
% \end{proof}

% We are now ready to prove Proposition \ref{mainrelax}.

% \begin{proof}
% The hypotheses imply that if $x$ is normal such that $W_i x = 0$ then
% \begin{equation}
% C \ \left| \left( g^{-1} \cdot W_i \right) \ x    \right|^n \leq |  \ \sigma(0) - \sigma ( W_i \ (g \cdot x) )   \ | < C \ \left( \frac{31}{256} \right)^{\frac{n}{2}}. 
% \end{equation}
% By Lemma \ref{lemmrelax} there exists $\rho_i(g) \in \textrm{U}(1) $ such that 
% \begin{equation}\label{ineqc}
% \| g^{-1} \cdot W_i - \rho_i(g) W_i \| < \sqrt{2\left( 1- \sqrt{1 -  \frac{31}{256 }} \right) } = \frac{\sqrt{2}}{4}.   
% \end{equation}



% In particular, $| \ W_{i,gh} - \rho_i(g)W_{i,h}   \  | < \frac{\sqrt{2}}{4} $ for all $g,h \in G$. Therefore, via the triangle inequality we see that 
% \begin{align}\label{ineqfinal}
% & | W_{i,g}W_{i,h} - W_{i,gh}  | \leq \\
% \leq & |W_{i,h} W_{i,g} - \rho_i(g) W_{i,h}| + | W_{i,gh} - \rho_i(g)W_{i,h} | = \\
% = &\bcancel{|W_{i,h}|} |W_{i,g} - \rho_i(g)W_{i,1}|  + | W_{i,gh} - \rho_i(g)W_{i,h} | < \frac{\sqrt{2}}{2}.
% \end{align}
% Equation \ref{ineqfinal} implies that $\| W_{\bullet , g} \odot W_{\bullet, h} - W_{\bullet,gh }  \| <  \frac{\sqrt{2d}}{2}$. Since $W$ is unitary, $\|  W_{\bullet, p}  - W_{\bullet, q}  \| = \sqrt{2d}$ for all $p \not = q \in G$. As a consequence, $W_{\bullet , g} \odot W_{\bullet, h}$ is closer to $W_{\bullet,gh}$ than to any other column of $W$, which immediately implies the desired result. 

% \end{proof}




% \subsection{Proof of Proposition \ref{prop:deepnets}}
% \begin{proof}
% Consider $W, W' \in \mathcal{W}$ such that $\varphi(W,x) = \varphi(W', x)$ for all $x \in \free{G}$. Given the open set $O \subseteq \mathbb{R}_{\geq 0}^k$ from the hypothesis on $\chi$, consider $O' = \{ x \in \free{G} \ | \ |Wx|^2, |W'x|^2 \in O \}$, which is open and non-empty since $0 \in O'$. For $x \in O'$, $\varphi(W,x)$ can be written as:
% \begin{equation}
% \varphi(W,x) = \sum_i a_i |W_i \ x|^2 + b,
% \end{equation}
% with the $a_i$'s being distinct, and similarly for $\varphi(W', x)$. Since Hermitian forms are determined by their restriction on an open set, we deduce the following identity of operators:
% \begin{equation}\label{eq:tensordense}
% \sum_i a_i W_i \otimes \overline{W_i} = \sum_i a_i W_i' \otimes \overline{W_i'}. 
% \end{equation}
% Since both the sets $\{ W_i\}_i$ and $\{ W_i'\}_i$ are orthonormal by hypothesis on $\mathcal{W}$, both sides of Equation \ref{eq:tensordense} define a spectral decomposition, i.e. a decomposition into projections over orthonormal vectors. Since the eigenvalues $a_i$ are distinct and non-vanishing, it follows that $W_i = \rho_i W_i'$ for some $\rho_i \in \textnormal{U}(\mathbb{C})$, as desired. 
% \end{proof}



% \begin{proof}
% Consider $W, W' \in \mathcal{W}$ such that $\varphi(W,x) = \varphi(W', x)$ for all $x \in \free{G}$. Given the open set $O \subseteq \mathbb{R}_{\geq 0}^k$ from the hypothesis on $\chi$, consider $O' = \{ x \in \free{G} \ | \ |Wx|^2, |W'x|^2 \in O \}$, which is open and non-empty since $0 \in O'$. For $x \in O'$, $\varphi(W,x)$ can be written as:
% \begin{equation}
% \varphi(W,x) = \sum_i a_i |W_i \ x|^2 + b,
% \end{equation}
% with the $a_i$'s being distinct, and similarly for $\varphi(W', x)$. Since Hermitian forms are determined by their restriction on an open set, we deduce the following identity of operators:
% \begin{equation}\label{eq:tensordense}
% \sum_i a_i W_i \otimes \overline{W_i} = \sum_i a_i W_i' \otimes \overline{W_i'}. 
% \end{equation}
% Since both the sets $\{ W_i\}_i$ and $\{ W_i'\}_i$ are orthonormal by hypothesis on $\mathcal{W}$, both sides of Equation \ref{eq:tensordense} define a spectral decomposition, i.e. a decomposition into projections over orthonormal vectors. Since the eigenvalues $a_i$ are distinct and non-vanishing, it follows that $W_i = \rho_i W_i'$ for some $\rho_i \in \textnormal{U}(\mathbb{C})$, as desired. 
% \end{proof}


% \begin{equation}\label{eq:tensordense}
% \sum_i a_i \  \partial_z \partial_{\overline{z}} \sigma(W_i \  x) \ W_i \otimes \overline{W_i} = \sum_i a_i \  \partial_z \partial_{\overline{z}} \sigma(W_i \  x) \ W_i' \otimes \overline{W_i'}. 
% \end{equation}
% Since both the sets $\{ W_i\}_i$ and $\{ W_i'\}_i$ are orthonormal by hypothesis on $\mathcal{W}$, both sides of Equation \ref{eq:tensordense} define a spectral decomposition for all $x$, i.e. a decomposition into projections over orthonormal vectors. Since $O'$ is an open set containing $0$, from orthogonality it follows that there exists $x \in O'$ such that all the $W_i \ x$'s coincide. Moreover, by hypothesis on $\sigma$, $x$ can be chosen such that $\partial_z \partial_{\overline{z}} \sigma(W_i \  x) \not = 0$. Therefore, the eigenvalues $a_i \  \partial_z \partial_{\overline{z}} \sigma(W_i \  x)$ of the operators in Equation \ref{eq:tensordense} are distinct and non-vanishing, implying that the eigenvectors have to coincide up to a multiplicative scalar i.e., $W_i = \rho_i W_i'$ for some $\rho_i \in \textnormal{U}(\mathbb{C})$, as desired. 
% \end{proof}


% \begin{equation}
% |\ \langle \widetilde{w}, x \rangle \ | = | \  \langle w, x \rangle   - \langle  w -  \widetilde{w}, x \rangle\ | \leq \varepsilon + \| \widetilde{w} - w \| = \varepsilon + \sqrt{2}. 
% \end{equation}


==> sections/0-abstract.tex <==
% [Principles for neural representation]. In this paper, we provide a theoretical explanation for [...] that is backed by the mathematical proof of the uniqueness of Fourier-based representations as a solution to the problem of invariant representation learning. [Tie to neuroscience and deep learning].

% Title: Learning Symmetry Groups from Data: The Power of Invariant Polyspectra

% We present a novel approach to learning symmetry groups from data based on invariant polyspectra. By leveraging the mathematical fact that all invariant polyspectra are unique, we demonstrate that a simple feedforward network that computes the power spectrum from a learned irreducible representation weight matrix can serve as a complete invariant map, with the same solution as more complex methods. This allows for the efficient construction of bispectral networks, which exhibit superior computational efficiency and learning properties. Compared to other methods for learning groups from data, which require expensive inference routines and lack algorithmic guarantees, our proposed approach offers the simplest, fastest, and most rigorous solution to date. These findings pave the way for scalable and efficient learning of more complex symmetry groups from data, with potential applications in fields such as computer vision and machine learning.


% In this work, we present a significant extension of our previous research on group-invariant learning using bispectra. Specifically, we prove that all invariant polyspectra are unique, which implies that the unique group-invariant polynomial can be constructed from the irreducible representations of the group, regardless of the degree of the spectrum. This mathematical fact has profound algorithmic implications, as we can design a simple network that computes the power spectrum from a learned irrep weight matrix as its invariant map, achieving the same result as much more expensive or complex methods. Moreover, using the learned irrep solution from the power spectral network, we can construct bispectral networks that are complete invariant maps, with significantly better scaling and learning properties. Our proposed method is the simplest, fastest, and most rigorous approach to learning symmetry groups from data, with algorithmic guarantees and complete invariance.



%cjh suggestions
In this work, we formally prove that, under certain conditions, if a neural network is invariant to a finite group then its weights recover the Fourier transform on that group. This provides a mathematical explanation for the emergence of Fourier features -- a ubiquitous phenomenon in both biological and artificial learning systems. The results hold even for non-commutative groups, in which case the Fourier transform encodes all the irreducible unitary group representations. Our findings have consequences for the problem of symmetry discovery. Specifically, we demonstrate that the algebraic structure of an unknown group can be recovered from the weights of a network that is at least approximately invariant within certain bounds. Overall, this work contributes to a foundation for an algebraic learning theory of invariant neural network representations. 

%This suggests that invariance is a powerful proxy objective for the problem of symmetry discovery
% \textit{convergent learning}

% previous: 
%In this work, we formally prove that if a neural network\footnote{of a certain kind; defined in Section \ref{sec:specnet}.} is invariant to a finite group, then its weights approximate a Fourier transform on that group. Emergent Fourier features are ubiquitous in both biological and artificial neural networks\textemdash a classic example of the broader phenomenon of \textit{convergent learning}. Our work is the first, to our knowledge, that provides a mathematical explanation for this phenomenon. Our work also has consequences for the problem of symmetry discovery; we demonstrate that the algebraic structure of an unknown group can be recovered from the weights of a neural network that has learned to be invariant to a group, so long as the model is within [... of ...]. This suggests that invariance is a powerful proxy objective for the problem of symmetry discovery. Our results hold for both commutative and non-commutative groups and set a foundation for a learning theory of neural network representations. 

% and is the first work, to our knowledge, to provide a mathematical explanation for this class of convergent learning phenomena.

% The \textit{universality hypothesis} states that models learn similar, ``universal,'' features when trained 

==> sections/1-introduction-v2.tex <==
% \begin{figure}[H]
%     \centering
%     {\transparent{.9}
%     \includegraphics[width=1.\textwidth]{figs/weights_rot.png}
%     \includegraphics[width=1.\textwidth]{figs/weights_trans.png}
%     }
% \caption{Weights of an invariant Power-Spectral Network trained on the MNIST dataset acted upon by the cyclic group $C_6 \simeq C_2 \times C_3$ via rotations (top) and via cyclic translations (bottom). }\label{fig:feature-examples}
% \end{figure}


\section{Introduction and Related Work}

% A notable and to-date unexplained phenomenon within deep learning theory is that of 

% The phenomenon of \textit{convergent learning} \cite{li2015convergent} is a notable property of deep learning. 

% \textit{Convergent learning} \cite{li2015convergent} or \textit{universality} \cite{olah2020overview}

% cjh suggestion:
Artificial neural networks trained on natural data exhibit a striking phenomenon: regardless of exact initialization, dataset, or training objective, models trained on the same data domain frequently converge to similar learned representations \cite{li2015convergent}. For example, the early layer weights of diverse image models tend to converge to Gabor filters and color-contrast detectors \cite{olah2020overview}. Remarkably, many of these same features are observed in the visual cortex \cite{hubel1959receptive, hass2013v1, willeke2023deep}, suggesting a form of representational \emph{universality} that transcends biological and artificial substrates. While such findings are empirically well-established \cite{rauker2023toward}, the field lacks theoretical explanations.

% prev:
%Artificial neural networks trained on natural data exhibit a striking phenomenon: regardless of exact initialization, dataset, or training objective, models trained on the same data domain frequently converge to similar learned representations \cite{li2015convergent}. For example, the early layer weights of diverse image models tend to converge to Gabor filters and color-contrast detectors \cite{olah2020overview}. Remarkably, many of these same features are observed in the visual cortex \cite{hubel1959receptive, hass2013v1, willeke2023deep}, suggesting a form of \textit{representational universality} that transcends biological and artificial substrate. While such findings are empirically well-established in the \textit{mechanistic interpretability} literature \cite{rauker2023toward}, the field still lacks theoretical explanation.

% A suite of results in the field of \textit{mechanistic interpretability} \cite{rauker2023toward} aims to reverse-engineer the weights of trained machine learning models. A suite of results in this direction has uncovered regularities for emergent features in artificial neural networks \cite{conmy2023towards}. Although these phenomena are empirically well-established, the field still lacks theoretical explanation.

Spatially localized versions of canonical 2D Fourier basis functions, such as Gabor filters or wavelets, are perhaps the most frequently observed universal features in image models. They commonly arise in the early layers of vision models -- trained with efficient coding \cite{olshausen1997sparse, bell1997independent}, classification \cite{olah2020overview}, temporal coherence \cite{hurri2003simple}, and next-step prediction \cite{fiquet2023polar} objectives --  as well as in the primary visual cortices of diverse mammals -- including cats \cite{hubel1962receptive}, monkeys \cite{hubel1968receptive}, and mice \cite{drager1975receptive}. Non-localized Fourier features have been observed in networks trained to solve tasks that permit cyclic wraparound -- for example, modular arithmetic \cite{nanda2023progress}, more general group compositions \cite{chughtai2023toy}, or invariance to the group of cyclic translations \cite{sanborn2023bispectral}. In the domain of spatial navigation, the so-called \textit{grid cells} of the entorhinal cortex \cite{moser2008place} display periodic firing patterns at different spatial frequencies as they build a map of space. Their response properties are naturally modeled with the harmonics of the twisted torus \cite{guanella2007model, orchard2013does, gardner2022toroidal}. Similar features also emerge in artificial neural networks trained to solve spatial navigation tasks \cite{banino2018vector, cueva2018emergence, sorscher2019unified, dorrell2022actionable, sorscher2023unified, schaeffer2023self}. The ubiquity of these features across diverse learning systems is both striking and unexplained.


In this work, we provide a mathematical explanation for the  emergence of Fourier features in learning systems such as neural networks. We argue that the mechanism responsible for this emergence is the downstream \textit{invariance} of the learner to the action of a \textit{group of symmetries} (e.g. planar translation or rotation). Since natural data typically possess symmetries, invariance is a fundamental bias that is injected both implicitly and sometimes explicitly into learning systems \cite{bronstein2021geometric}. Motivated by this, we derive theoretical guarantees for the presence of Fourier features in invariant learners that apply to a broad class of machine learning models. 

Our results rely on the inextricable link between harmonic analysis and group theory \cite{folland2016course}. The standard discrete Fourier transform is a special case of more general Fourier transforms on groups, which can be defined by replacing the standard basis of harmonics by irreducible unitary group representations. The latter are equivalent to the familiar definition for cyclic or, more generally, commutative groups, but are more involved for non-commutative ones. In order to accommodate both the scenarios, we develop a general theory that applies, in principle, to arbitrary finite groups. 

% cjh suggestion
This work represents an attempt to provide mathematical grounding for a general algebraic theory of representation learning, while addressing the \textit{universality hypothesis} for neural networks \cite{olah2020overview, moschella2022relative}. A suite of earlier theoretical works \cite{isely2010deciphering, hillar2015can, garfinkle2019uniqueness} established such universality for sparse coding models \cite{olshausen1997sparse}, deriving the conditions under which a network will recover the original bases that generate data through sparse linear combinations. In this case, the statistics of the data determine the uniqueness of the representation. Our findings, on the other hand, are purely \textit{algebraic}, since they rely exclusively on the invariance properties of the learner. Given the centrality of invariance to many machine learning tasks, our theory encompasses a broad class of scenarios and neural network architectures, while providing a new perspective on classical neuroscience \cite{pitts1947we, hubel1962receptive}. As such, it sets a foundation for a learning theory of representations in artificial and biological neural systems, grounded in the mathematics of symmetry.

% prev: 
%This work represents a significant attempt to provide theoretical grounding for the phenomenon of convergent learning (i.e. the \textit{universality hypothesis} \cite{olah2020overview, moschella2022relative}). A suite of earlier theoretical works \cite{isely2010deciphering, hillar2015can, garfinkle2019uniqueness} tackled a related problem, establishing guarantees that a model will recover (up to scaling) the true underlying basis of data generated as a sparse linear combination of those bases. Our findings here suggest [...] Given the centrality of invariance to many machine learning tasks, our proof is able to explain a broad class of convergent learning phenomena, in a broad class of neural network architectures, while providing a new perspective on classical neuroscience results. As such, it sets a foundation for a learning theory of representations in artificial and biological neural systems, grounded in the mathematics of symmetry.

 % any network that accurately encodes sparse linear combinations of a given set of basis functions recovers those bases up to scaling \cite{hillar2015can, garfinkle2019uniqueness}, a finding leveraged for an unsupervised communication model between brain regions \cite{isely2010deciphering}. More generally,

 % it sets a foundation for future work in mechanistic interpretability, opening the door for further mathematical explanation of the emergence of universal features in artificial and biological learning systems. 
 
 
 % In particular, we focus on the emergence of \textit{Fourier features} in artificial neural networks, and are able to derive a theoretical guarantee for the emergence of these features in models trained on tasks that require \textit{invariance} or \textit{equivariance} to the actions of a \textit{group of transformations} (e.g. planar translation or rotation). 




% The standard Fourier transform is a special case of more general Fourier transforms on groups \cite{rudin1964fourier}, which can be defined by replacing the standard Fourier basis\textemdash equivalent to the irreducible representations of the group of cyclic translations\textemdash with the irreps of other compact groups. For example, Fourier transforms can be defined on the groups of 2D and 3D rotation using the bases of disk harmonics or spherical harmonics. Notably, these more general Fourier features have been observed to emerge in neural networks trained on tasks that require invariance or equivariance to different groups \cite{sanborn2023bispectral, fiquet2023polar}, and have been suggested as an explanation for features observed throughout the mammalian visual cortex \cite{}. 

% \footnote{Mathematically, the Fourier transform is a projection of a signal onto the \textit{irreducible representations} of a group\textemdash cyclic translation in the standard case. This gives it the property of \textit{equivariance} to the group. Fourier transforms can be defined on other groups by replacing the standard Fourier basis with other irreducible group representations. For example, the disk harmonics or spherical harmonics can be used to define Fourier transforms on the groups $SO(2)$ and $SO(3)$ or 2D and 3D rotations.} 

% In this paper, we explain the emergence of both localized and general group-Fourier features in neural networks.

% In this paper, we suggest that these empirical observations may be explained by the ubiquity of \textit{invariance} and \textit{equivariance} in the structure of many tasks relevant for perception and intelligence. Our proof [...]. Concretely, our contributions are as follows:

% \begin{itemize}
%     \item We prove that if a neural network of a certain kind is invariant to a group $G$, then its weights must (almost) coincide with the irreducible unitary representations of that group.
%     \item Our proof covers both commutative and non-commutative groups, and a general class of neural network architectures, including convolutional networks and multi-layer perceptrons with [...] activation functions, including [...] and polynomial activations. 
%     \item We demonstrate this convergent learning in a suite of empirical experiments, and show that across initializations, on a diverse set of datasets and network architectures, models consistently converge to the theoretically predicted representations.
% \end{itemize}

\subsection{Overview of Results}\label{sec:overview}
In this section, we provide a non-technical overview of the theoretical results presented in this work. Our main result can be summarized as follows.  
\begin{infthm}[Theorem \ref{prop:mainnew} and Corollary \ref{mainpropnc}]\label{thm:mainintui}
If $\varphi(W,x)$ is a parametric function of a certain kind that is invariant in the input variable $x$ to the action of a finite group $G$, then each component of its weights $W$ coincides with a harmonic of $G$ up to a linear transformation. In particular, when the weights are orthonormal, $W$ coincides with the Fourier transform of $G$ up to linear transformations. 
\end{infthm}
In the above, the term `harmonic' refers to an irreducible unitary representation of $G$. Indeed, one-dimensional unitary representations correspond to homomorphisms with the unit circle $\textnormal{U}(1) \subseteq \mathbb{C}$, which is reminiscent of the classical definition via the imaginary exponential. However, \emph{non-commutative} groups can have higher-dimensional irreducible representations, intuitively meaning that harmonics are valued in unitary matrices. In this case, the components of $W$ can be interpreted as \emph{capsules} in the sense of \cite{hinton2018matrix} i.e., neural units processing matrix-valued signals. 


We show that the hypothesis on $\varphi$ in Theorem \ref{thm:mainintui} is satisfied by several machine learning models from the literature. In particular, the theorem applies to the recently-introduced (Bi)Spectral Networks \cite{sanborn2023bispectral} and, to an extent, to more traditional learners, including fully-connected McCulloch-Pitts neurons, deep networks, and self-attention mechanisms. Since harmonic analysis is naturally formalized over the complex numbers, we consider models with complex weights $W$, which fits into the larger program of complex-valued machine learning \cite{bassey2021survey, trabelsi2017deep, lowe2022complex}. 


The group-theoretical Fourier transform encodes the entire group structure of $G$. Therefore, as a consequence of Theorem \ref{thm:mainintui} the multiplication table of $G$ can be recovered from the weights $W$ of an invariant parametric function $\varphi$ -- a fact empirically demonstrated in \cite{sanborn2023bispectral}. This  addresses the question of \emph{symmetry discovery} -- an established machine learning problem aiming to recover the unknown group of symmetries of data with minimal supervision and prior knowledge \cite{rao1998learning, sohl2010unsupervised, desai2022symmetry}.

Since the multiplication table is a discrete object, it is expected that the invariance constraint on $\varphi$ can be loosened while still recovering the group correctly. To this end, we prove the following. 

\begin{infthm}[Theorem \ref{prop:mainrelax}]\label{thm:boundsintui}
If $\varphi(W,x)$ is `almost invariant' to $G$ according to certain functional bounds and the weights are `almost orthonormal', then the multiplicative table of $G$ can be recovered from $W$. 
\end{infthm}

Lastly, we implement a model satisfying the requirements of our theory and demonstrate its symmetry discovery capabilities. To this end, we train it via contrastive learning on an objective encouraging invariance and extract the multiplicative table of $G$ from its weights. Our Python implementation is available at a public repository \footnote{\url{https://github.com/sophiaas/spectral-universality}}.       

%A central feature of the canonical Fourier transform is that it is \textit{equivariant} to the group of cyclic translations. This arises from the fact that the Fourier transform is a projection of a signal onto the set of \textit{irreducible representations} of this group. Fourier transforms can be more generally defined on other compact groups, by replacing the standard Fourier basis with the irreducible representations of other groups \cite{rudin1964fourier}.

% Notably, these features have been empirically observed in many network architectures trained on diverse tasks. For example, Fourier features emerge in a one-layer ReLU Network trained to solve modular arithmetic \cite{nanda2023progress}, [...], and in a complex-valued polynomial neural network trained to output invariant representations \cite{sanborn2023bispectral}. 

% Spatially localized versions of canonical 2D Fourier basis functions (i.e. Gabor filters or wavelets) are commonly observed in early layers of both biological and artificial neural networks\textemdash appearing in vision models trained with efficient coding \cite{olshausen1997sparse, bell1997independent}, classification \cite{olah2020overview}, temporal coherence \cite{hurri2003simple}, and next-step prediction \cite{fiquet2023polar} objectives, as well as in the primary visual cortices of cats, monkeys, mice, and humans \cite{hubel1959receptive}. 

 % Restricting ourselves to the problem of \textit{invariant representation learning}, we are able to derive a theoretical guarantee for the emergence of certain features in the learned weight matrices of artificial networks. In particular, we prove that networks trained to be invariant to the actions of a \textit{group of transformations} (e.g. planar translation or rotation) will learn the irreducible representations of that group (i.e. group-Fourier features: the 2D Fourier basis for planar translation, or the disk harmonics for planar rotation). 


% Fourier features (i.e. irreducible group representations). 

% The conditions we restrict ourselves to are the natural 

% In particular, we restrict ourselves to the problem of \textit{invariant representation learning} and derive a theoretical guarantee for the emergence of Fourier features (i.e. irreducible group representations). 

% in the context of invariant representation learning. 

% One notable regularity across tasks is the emergence of Fourer  In this paper, we prove theoretical proof guaranteeing convergent learning in the context of invariant representation learning. In particular, we are


% Remarkably, there are striking consistencies in the neural features that emerge in both artificial and biological systems trained to solve similar tasks.
% % % Across neural systems trained to solve vision tasks\textemdash artificial and biological alike\textemdash there is a striking regularity in the features that emerge.
% For example, in the primary visual cortex, so-called \textit{simple cells} are selective for localized Fourier features \cite{hubel1959receptive, kulikowski1982theory}. Surprisingly, these very same features emerge in artificial neural networks trained to solve vision tasks, including compression \cite{olshausen1997sparse, bell1997independent} and image classification
% \cite{olah2020overview}. This consistency can be observed across neural networks with different architectures and random initializations, trained on [similar but non-identical data]. 

% % For example, in the primary visual cortex, so-called \textit{simple cells} are selective for bars of certain spatial frequencies and orientations \cite{hubel1959receptive}. The response properties of these neurons can be modeled with Gabor wavelets \cite{kulikowski1982theory}\textemdash localized 2D Fourier filters. 

% One explanation for the so-called \textit{universality} \cite{olah2020overview} of these features is provided by the \textit{efficient coding hypothesis}, which proposes that biological brains\textemdash being fundamentally resource-constrained\textemdash have evolved to optimally compress information. Several of the features observed in the early visual system can be derived as optimal and unique \cite{isely2010deciphering, garfinkle2019uniqueness} solutions to the compression problem, given the statistics of natural data \cite{simoncelli2001natural, dan1996efficient, olshausen1997sparse, bell1997independent}. This provides an explanation for why these features appear in artificial networks trained to solve compression tasks. However, it remains mysterious why the same features emerge in the early layers of image classification models, which have no explicit compression objective. [Indeed, compression can't be the whole story. Even the biggest proponent of the efficient coding theory later revised the perspective to state that the \textit{utility} of representations for downstream computation is more important \cite{barlow2001redundancy}. ]

% Intriguingly, Fourier-based features are not only observed in the context of vision. The periodic firing patterns of grid cells in the entorhinal cortex\cite{moser2008place}\textemdash the seat of the brain's spatial navigation system\textemdash can also be understood as [the eigenvectors of the successor representation] \cite{stachenfeld2017hippocampus} or the [positive-only harmonics of the torus \cite{gardner2022toroidal}, the compactified plane]. Fourier features have also been observed to emerge in artificial neural networks trained to solve arithmetic tasks \cite{nanda2023progress} and [... more diverse citations!]


% How is information represented by populations of neurons in the brain? Are there general principles underlying this process\textemdash laws of neural representation? In this paper, we use techniques from algebraic geometry and theorems fundamental to invariant theory \cite{sturmfels2008algorithms} to derive a novel principle for neural coding. Our proofs provide a unification of foundational results in both deep learning and neuroscience, explaining the convergent emergence of Fourier-based features in biological and artificial neural systems as a unique and thus universal solution to the problem of invariant representation learning.


%[Modeling transformation structure is essential for intelligence]. [The transformation structure of the natural world is described by groups]. [Fourier features are tied to groups as they are irreps]. Concretely, we demonstrate that Fourier solutions are guaranteed to emerge in neural systems trained to form group-invariant representations of inputs. [Polynomial assumption]. 


% Our results have profound implications for neuroscience theory and deep learning theory alike. From the side of neuroscience, our results provide novel theoretical explanations for existing neuroscience data and new predictions that could guide novel experimental neuroscience research. [Tie in mathematics]. From the side of deep learning theory, our results provide novel guarantees for [expected neural representations], a [rare contribution] to the field of interpretability research. 

==> sections/1-introduction.tex <==

\begin{figure}[H]
    \centering
    {\transparent{.9}
    \includegraphics[width=1.\textwidth]{figs/weights_rot.png}
    \includegraphics[width=1.\textwidth]{figs/weights_trans.png}
    }
    \caption{Weights of an invariant Power-Spectral Network trained on the MNIST dataset acted upon by the cyclic group $C_6 \simeq C_2 \times C_3$ via rotations (top) and via cyclic translations (bottom). }
    \label{fig:feature-examples}
\end{figure}

% The ability to form \textit{invariant representations} is central to intelligence. Invariance plays a fundamental role in many deep learning algorithms. Despite this, few papers in the field have made use of the rich set of mathematical tools provided by invariant theory and algebraic geometry \cite{sturmfels2008algorithms}. In this paper, we use techniques from algebraic geometry and theorems fundamental to invariant theory to provide novel guarantees regarding neural network solutions to invariant representation learning. 


%---------------------

% 1. Formal result (commutatibe and non-commutative) on bispectral / spectral networks
% 2. Semi-formal result on transformers
% 3. Empirical discussionon piecewise linear networks
% 4. Empirical results for local translations (Gabors)

% Transformer relationship to bispectral networks. Mean over the first two terms, minimum over the last (softmax)

% Train a transformer on the invariance problem (rotated mnist)

% {\color{red}Desiderata: 
% \begin{itemize}
% \item Radius of recovery of the Cayley table.
% \item Locality: do local symmetries give the same result for local Fourier features i.e., Gabor filters?
% \item Connection between self-attention mechanisms (e.g., Visual Transformers) and Bispectral Networks. The softmax requires special care.  
% \end{itemize}


% }

% \section{Introduction}

% This work is supported by the results of a recent paper, \textit{Bispectral Neural Networks} \cite{sanborn2023bispectral}, which demonstrates that irreducible representations can be learned in a third-order neural network that mirrors the ansatz of the bispectrum. Indeed, our theoretical results guarantee this solution. Moreover, they motivate the proposal of a new neural network architecture, which we call \textit{Power Spectral Networks}

% [In a way, we are answering a question first raised by the inventors of the first neural network in 1947 in a remarkable piece title \textit{How We know Universals} \cite{pitts1947we}\textemdash the first work we are aware of to tie neural networks to group theory for the problem of solving invariant representation learning.] 

% The ability to form \textit{invariant representations} is central to intelligence. Invariance plays a fundamental role in many deep learning algorithms. Despite this, few papers in the field have made use of the rich set of mathematical tools provided by invariant theory and algebraic geometry \cite{sturmfels2008algorithms}. In this paper, we use techniques from algebraic geometry and theorems fundamental to invariant theory to provide novel guarantees regarding neural network solutions to invariant representation learning. 

% Previous Bispectrum Introduction
\section{Introduction}
% The \textit{symmetries} of perception define the transformations that can be performed in the world that are not meaningful for a task and leave the agent's interpretation invariant. 

% symmetries of the natural world.
% \vspace{-0.2cm}
% A fundamental problem of intelligence is to model the transformation structure of the natural world.  In the context of vision, translation, rotation, and scaling define symmetries of object categorization\textemdash the transformations that leave perceived object identity invariant. In audition, pitch and timbre define symmetries of speech recognition. Biological neural systems have learned these symmetries from the statistics of the natural world\textemdash either through evolution or accumulated experience. Here, we tackle the problem of learning symmetries in artificial neural networks. 

% At the heart of the challenge lie two requirements that are frequently in tension: \textit{invariance} to transformation structure and \textit{selectivity} to pattern structure. In deep networks, operations such as \texttt{max} or \texttt{average} are commonly employed to achieve invariance to local transformations. Such operations are invariant to many natural transformations; however, they are also invariant to unnatural transformations that destroy image structure, such as pixel permutations. This lack of selectivity may contribute to failure modes such as susceptibility to adversarial perturbations \cite{goodfellow2014explaining}, excessive invariance \cite{jacobsen2018excessive}, and selectivity for textures rather than objects \cite{brendel2019approximating}. Thus, there is a need for computational primitives that selectively parameterize natural transformations and facilitate robust invariant representation learning.

% An ideal invariant would be \textit{complete}. A complete invariant preserves all pattern information and is invariant only to specific transformations relevant to a task. Transformations in many datasets arise from the geometric structure of the natural world. The mathematics of \textit{groups} and their associated objects give us the machinery to precisely define, represent, and parameterize these transformations, and hence the problem of invariant representation learning. In this work, we present a novel neural network primitive based on the \textit{bispectrum}, a complete invariant map rooted in harmonic analysis and group representation theory \cite{kakarala1993group}. 

% % A \textit{complete} invariant map is selective: it preserves all pattern information and is invariant only to specific transformations relevant to a task. 

% Bispectral Neural Networks flexibly parameterize the bispectrum for arbitrary compact commutative groups, enabling both the group and the invariant map to be learned from data. The architecture is remarkably simple. It is comprised of two layers: a single learnable linear layer, followed by a fixed collection of triple products computed from the output of the previous layer. BNNs are trained with an objective function consisting of two terms: one that collapses all transformations of a pattern to a single point in the output (invariance), and another that prevents information collapse in the first layer (selectivity). 

% % Critically, \textit{the model generalizes to novel, out-of-distribution classes}
%  We demonstrate that BNNs trained to separate orbit classes in augmented data learn the group its Fourier transform, and corresponding bispectrum purely from the symmetries implicit in the data (Section \ref{section:learningirreps}). Because the model has learned the fundamental structure of the group, we show that it generalizes to novel, out-of-distribution classes with the same group structure and facilitates downstream group-invariant classification (Section \ref{section:classification}). Further, we demonstrate that the trained network inherits the completeness of the analytical model, which endows the network with strong adversarial robustness (Section \ref{section:adversarial}). Finally, we demonstrate that the weights of the network can be used to recover the group Cayley table\textemdash the fundamental signature of a group's structure (Section \ref{section:cayley}). Thus, an explicit model of the group can be learned and extracted from the network weights. To our knowledge, our work is the first to demonstrate that either a bispectrum or a group Cayley table can be learned from data alone. Our results set the foundation of a new computational primitive for robust and interpretable representation learning.



% There have been many attempts in the literature to discover latent group structure in data. [1,2,3] The different methods frequently make use of the notion of irreducible representations of groups to parameterize models which can learn, in a semi-supervised or unsupervised manner, the irreps corresponding to the underlying group structure from variations in data alone. 
% However, the proposed methods suffer from notable drawbacks / have notable limitations. First, they are computationally expensive to compute, invoking either bayesian inference and MAP estimation using the exponential map.

% Our previous work on bispectral neural networks demonstrates that there is a \textit{complete} invariant map which can be computed with a single feedforward map in a higher-order neural network architecture which parameterizes the ansatz of the solution. We have shown in prior work that, with a simple, principled contrastive training strategy, the model converges to the ground truth irreducible representations, and thus, has learned the group. However, at the time there were no formal guarantees as to the \textit{uniqueness} of the bispectral solution, despite the fact that the network converged to this solution. 

% A recent discovery by Giovanni and our team has shown that, for CCC groups, the n-spectra are the unique polynomial invariants for all n (greater than or equal to 2). This means that, indeed, the bispectrum/irreps are a unique solution to the problem posed in the previous paper. However, the theorem has a second, resounding \textit{algorithmic} implication. In particular, it implies that the power spectrum solution is also a unique solution, and, given that the power spectrum is defined in terms of the same irreducible representations, this means the group structure can be discovered by instead simply parameterizing the ansatz of the 2-spectrum. After training, the irreps can be used to construct the third-order complete invariant, namely, the bispectrum.

% This is significant, as the power spectrum computation scales linearly as a function of input dimension, whereas the bispectrum (naively) scales as $n^2$.





% Furthermore, as the power spectrum is quadratic in the signal energies, ...
% perhaps make a comment about the loss landscape of the power spectral net vs the bispectral net? 
    %This was unclear in the cubic case of the bispectrum. 

% In this work, we prove the uniqueness of the n-spectra and demonstrate a resulting simple, efficient architecture which learns the irreducible representations from data with strong mathematical guarantees.

% % How is information represented by populations of neurons in the brain? Are there general principles underlying this process\textemdash laws of neural representation? In this paper, we use techniques from algebraic geometry and theorems fundamental to invariant theory \cite{sturmfels2008algorithms} to derive a novel principle for neural coding. Our proofs provide a unification of foundational results in both deep learning and neuroscience, explaining the convergent emergence of Fourier-based features in biological and artificial neural systems as a unique and thus universal solution to the problem of invariant representation learning.

% This work is supported by the results of a recent paper, \textit{Bispectral Neural Networks} \cite{sanborn2023bispectral}, which demonstrates that irreducible representations can be learned in a third-order neural network that mirrors the ansatz of the bispectrum. Indeed, our theoretical results guarantee this solution. Moreover, they motivate the proposal of a new neural network architecture, which we call \textit{Power Spectral Networks}
% % In this paper, we tackle the question of universality from the perspective of group theory. 
% From the side of deep learning theory, our results provide novel guarantees for [expected neural representations], a [rare contribution] to the field of interpretability research. 


% % not true: nix this: Furthermore, as the power spectrum is quadratic in the signal energies, perhaps we can show that the loss function is in fact \textit{convex} when restricted to the set of matrices which are permutation equivalent to an orthonormal basis. 
% % This would mean that we would be guaranteed that there is a global minimum (up to permutation) and a convex landscape allowing it to be reached by the algorithm.

% -----------


% \label{sec:introduction}

% Bispectrum + Transformers relationship

% COMMENTS FROM CHRIS:
% Invariant theory and polynomial algebra has a surprising role to play in this problem, we're able to use concepts from pure mathematics to make profound statements about neural representations.
% We're also using unique factorization of polynomials
% For gabors: local translations
% For grid cells, subgroups of 2d cyclic translation

%%%%%%%%%%%%%
% VERSION 1 % 
%%%%%%%%%%%%%

% Neurons in artificial neural networks were originally inspired by the ``feature detector'' model of biological neurons: The classic idea from visual neuroscience that single neurons identify the presence of certain structured information in the environment\textemdash for example, an edge in a region of a visual scene \cite{hubel1959receptive}. 

% This idea inspired the development of the first convolutional neural network architectures \cite{fukushima1980neocognitron} and remains a dominant paradigm for information representation in artificial neural networks today.

% At the intersection of neuroscience and deep learning, there lies a long-standing puzzle: Why are similar features observed in both biological brains and artificial neural networks? Why are similar features observed across different brains? Across different artificial neural networks? Is there something fundamental about certain features\textemdash a certain ``universality''? 

% [How we know universals]



% A classical perspective in neuroscience is that single neurons function as ``feature detectors'' that identify the presence of certain structured information in the environment \cite{barlow1972single}\textemdash for example, an edge in a region of a visual scene \cite{hubel1959receptive}. The firing rate of a neuron is thought to reflect ``how much'' of that feature is present in the input. This idea inspired the development of the first convolutional neural network architectures \cite{fukushima1980neocognitron} and remains a dominant paradigm for information representation in artificial neural networks today. 

% A classical perspective in neuroscience is that single neurons function as ``feature detectors'' that identify the presence of certain structured information in the environment \cite{barlow1972single}\textemdash for example, an edge in a region of a visual scene \cite{hubel1959receptive}. The firing rate of a neuron is thought to reflect ``how much'' of that feature is present in the input\textemdash i.e. how good of a match the neuron's receptive field is to the data. This idea inspired the development of the first convolutional neural network architectures \cite{fukushima1980neocognitron} and remains a dominant paradigm for information representation in artificial neural networks today. 

% Remarkably, there are striking consistencies in the neural features that emerge in both artificial and biological systems trained to solve similar tasks.
% % % Across neural systems trained to solve vision tasks\textemdash artificial and biological alike\textemdash there is a striking regularity in the features that emerge.
% For example, in the primary visual cortex, so-called \textit{simple cells} are selective for localized Fourier features \cite{hubel1959receptive, kulikowski1982theory}. Surprisingly, these very same features emerge in artificial neural networks trained to solve vision tasks, including compression \cite{olshausen1997sparse, bell1997independent} and image classification
% \cite{olah2020overview}. This consistency can be observed across neural networks with different architectures and random initializations, trained on [similar but non-identical data]. 

% % For example, in the primary visual cortex, so-called \textit{simple cells} are selective for bars of certain spatial frequencies and orientations \cite{hubel1959receptive}. The response properties of these neurons can be modeled with Gabor wavelets \cite{kulikowski1982theory}\textemdash localized 2D Fourier filters. 

% One explanation for the so-called \textit{universality} \cite{olah2020overview} of these features is provided by the \textit{efficient coding hypothesis}, which proposes that biological brains\textemdash being fundamentally resource-constrained\textemdash have evolved to optimally compress information. Several of the features observed in the early visual system can be derived as optimal and unique \cite{isely2010deciphering, garfinkle2019uniqueness} solutions to the compression problem, given the statistics of natural data \cite{simoncelli2001natural, dan1996efficient, olshausen1997sparse, bell1997independent}. This provides an explanation for why these features appear in artificial networks trained to solve compression tasks. However, it remains mysterious why the same features emerge in the early layers of image classification models, which have no explicit compression objective. [Indeed, compression can't be the whole story. Even the biggest proponent of the efficient coding theory later revised the perspective to state that the \textit{utility} of representations for downstream computation is more important \cite{barlow2001redundancy}. ]

% Intriguingly, Fourier-based features are not only observed in the context of vision. The periodic firing patterns of grid cells in the entorhinal cortex\cite{moser2008place}\textemdash the seat of the brain's spatial navigation system\textemdash can also be understood as [the eigenvectors of the successor representation] \cite{stachenfeld2017hippocampus} or the [positive-only harmonics of the torus \cite{gardner2022toroidal}, the compactified plane]. Fourier features have also been observed to emerge in artificial neural networks trained to solve arithmetic tasks \cite{nanda2023progress} and [... more diverse citations!]

% In this paper, we offer a new perspective on universality that is grounded in group theory. [connect the notion of usefulness of representations to equivariance]. A common factor shared by all the tasks described is the importance of modeling \textit{transformations}

% [Cite recent universality group learning paper  \cite{chughtai2023toy}]

% The primary contributions of this work are [...]


% [In a way, we are answering a question first raised by the inventors of the first neural network in 1947 in a remarkable piece title \textit{How We know Universals} \cite{pitts1947we}\textemdash the first work we are aware of to tie neural networks to group theory for the problem of solving invariant representation learning.] 

% This work is supported by the results of a recent paper, \textit{Bispectral Neural Networks} \cite{sanborn2023bispectral}, which demonstrates that irreducible representations can be learned in a third-order neural network that mirrors the ansatz of the bispectrum. Indeed, our theoretical results guarantee this solution. Moreover, they motivate the proposal of a new neural network architecture, which we call \textit{Power Spectral Networks}



% that provide an optimal basis for [successor representation]].



% that they reflect the statistical structure of natural signals \cite{simoncelli2001natural}. For example, the Fourier-based filters that commonly emerge in the early layers of deep networks are mathematically guaranteed as a [unique optimally sparse code of natural images] \cite{isely2010deciphering, garfinkle2019uniqueness}.

% permit the sparse \cite{olshausen1997sparse}, factorized \cite{bell1997independent} representation of natural images. Indeed, these features are mathematically guaranteed as a unique solution to the sparse coding problem on these data \cite{isely2010deciphering, garfinkle2019uniqueness}. 

% \cite{chughtai2023toy} \cite{nanda2023progress}

% One explanation for this phenomenon is that the Gabor filter basis is intimately related to the statistical structure of natural images \cite{simoncelli2001natural}, as it permits the sparse \cite{olshausen1997sparse}, factorized \cite{bell1997independent} representation of these signals. Indeed, for natural images, the observed Gabor-like solution is mathematically guaranteed as a unique solution to the sparse coding problem \cite{isely2010deciphering, garfinkle2019uniqueness}. 

% [Statistics of natural signals cited as common explanation \cite{simoncelli2001natural}]. In the field of mechanistic interpretability research \cite{olah2020overview}, the \textit{universality hypothesis} [...]



% One explanation for this phenomenon is that the Gabor filter basis is intimately related to the statistical structure of natural images \cite{simoncelli2001natural}, as it permits the sparse \cite{olshausen1997sparse}, factorized \cite{bell1997independent} representation of these signals. Indeed, for natural images, the observed Gabor-like solution is mathematically guaranteed as a unique solution to the sparse coding problem \cite{isely2010deciphering, garfinkle2019uniqueness}. 

% Across artificial and biological neural systems trained on vision tasks, there are striking consistencies in the features that

% How is information represented by populations of neurons in the brain? Are there general principles underlying this process\textemdash laws of neural representation? In this paper, we use techniques from algebraic geometry and theorems fundamental to invariant theory \cite{sturmfels2008algorithms} to derive a novel principle for neural coding. Our proofs provide a unification of foundational results in both deep learning and neuroscience, explaining the convergent emergence of Fourier-based features in biological and artificial neural systems as a unique and thus universal solution to the problem of invariant representation learning.

% invariant representation learning in neural systems.

A classical perspective in visual neuroscience is that single neurons function as `feature detectors' that identify the presence of certain structured information in the world\textemdash for example, an edge in a region of a scene \cite{hubel1959receptive}. The firing rate of a neuron is thought to reflect `how much' of that feature is present in the input i.e., how good of a match the neuron's receptive field is to the data. This idea inspired the development of the first convolutional neural network architectures \cite{fukushima1980neocognitron} and remains the dominant paradigm for information representation in artificial neural networks today. 

Remarkably, there are striking consistencies in the features that emerge in both artificial and biological neural systems trained on vision tasks.
% Across neural systems trained to solve vision tasks\textemdash artificial and biological alike\textemdash there is a striking regularity in the features that emerge.
For example, in the primary visual cortex, so-called \textit{simple cells} are selective for bars of certain spatial frequencies and orientations \cite{hubel1959receptive}. The response properties of these neurons can be modeled with Gabor wavelets \cite{kulikowski1982theory}\textemdash localized 2D Fourier filters. Surprisingly, these very same features emerge in artificial neural networks trained to efficiently encode natural images \cite{olshausen1997sparse}, as well as deep convolutional networks trained to solve image classification problems \cite{olah2020overview}. One informal explanation for this phenomenon is that the Gabor/Fourier filter basis is intimately related to the statistical structure of natural images \cite{simoncelli2001natural}, as it permits the sparse \cite{olshausen1997sparse}, factorized \cite{bell1997independent} representation of these signals. While this explanation provides [good properties of the explanation], it lacks [things that are missing]. Fourier-based representations are not unique to vision. For example, the canonical grid cell representations observed in the brain's spatial navigation system \cite{moser2008place} [are Fourier based \cite{bush2015using}, eigenvectors of successor representations \cite{kulkarni2016deep, momennejad2018predicting, de2020neurobiological, stoewer2022neural}]. [Further explanation of grid cell phenomena]. [Twisted torus citation \cite{guanella2007model}]

% Moreover, Gabor features also emerge in neural network models that possess no sparsity constraint \cite{fiquet2023polar}

% Indeed, for natural images, the observed Gabor-like solution is mathematically guaranteed as a unique solution to the sparse coding problem \cite{isely2010deciphering, garfinkle2019uniqueness}.

In this work, we offer a mathematical explanation for the emergence of Fourier-based features in neural systems that makes use of the inextricable link between harmonic analysis and group theory. The Fourier transform is indeed rooted in the symmetry structure of the underlying space, and plays an essential role in the mathematical study of groups. Based on this, we argue that the fundamental property responsible for the emergence of Fourier features is \emph{invariance} to symmetries of data. Specifically, our main result shows that if a {\color{blue}certain class} of neural networks is invariant to a group of symmetries, then the associated weights must (almost) coincide with the Fourier transform of the underlying group. The result is general, with an algebraic proof which applies to both commutative as well as noncommutative groups. In the latter case the Fourier features are valued in (irreducible) unitary group representations, which can be interpreted as a version of vector neurons [ref for vector neurons]. 

Our findings have the following significant implication from a machine learning perspective. Since the Fourier transform encodes all the information about the underlying group up to isomorphism, a consequence of our results is that the group structure can be recovered from the weights of an invariant network. The recovery algorithm is simple and efficient. This  addresses the question of \emph{symmetry discovery} -- an established machine learning problem aiming to recover the (unknown) group of symmetries of data with minimal supervision and prior knowledge. We further analyze our group discovery algorithm from a numerical perspective. Namely, we provide a relaxation of the invariance condition under which the group is still recovered correctly, even though the network's weights are only approximately close to Fourier features. 




%[Modeling transformation structure is essential for intelligence]. [The transformation structure of the natural world is described by groups]. [Fourier features are tied to groups as they are irreps]. Concretely, we demonstrate that Fourier solutions are guaranteed to emerge in neural systems trained to form group-invariant representations of inputs. [Polynomial assumption]. 


% Our results have profound implications for neuroscience theory and deep learning theory alike. From the side of neuroscience, our results provide novel theoretical explanations for existing neuroscience data and new predictions that could guide novel experimental neuroscience research. [Tie in mathematics]. From the side of deep learning theory, our results provide novel guarantees for [expected neural representations], a [rare contribution] to the field of interpretability research. 


% Our contributions are summarized as follows: 
% \begin{itemize}
%     \item A theoretical result stating that the weights of a group-invariant complex neural network of a certain type (almost) coincide with the coefficients of the Fourier transform of the group. We prove the result for both commutative and noncommutative groups. 
%     \item An algorithm recovering the group structure from the weights of an invariant network, together with a relaxation of invariance under which the algorithm holds. 
%     \item An empirical investigation [...]. 
% \end{itemize}








% Indeed, given a particular dataset, there is a unique solution to the sparse coding problem \cite{garfinkle2019uniqueness}, which is the Gabor filter solution observed for natural image datasets. 


%%%%%%%%%%%%%%%%%
% VERSION 2 WIP % 
%%%%%%%%%%%%%%%%%

% The \textit{Fourier transform} and its spatial dual\textemdash the \textit{convolution}\textemdash are foundational to modern deep learning. Most in the field are familiar with the Fourier transform as a method for frequency decomposition and convolution as a method for feature detection. However, these operations owe much of their power to their lesser-known mathematical foundations in group theory: the mathematics of \textit{symmetries} and \textit{transformations}. 

% % Most in the field are familiar with the Fourier transform as a method for frequency decomposition and convolution as a method for feature detection. 

% An essential, if not defining, property of the Fourier transform is that it is a symmetry-preserving (\textit{equivariant}) map. This means that a transformation in the input space gives rise to a corresponding transformation in the output space. [This gives it special properties that can be exploited]. The standard Fourier transform is equivariant to \textit{translations} in the input, which result in phase shifts on the Fourier coefficients\textemdash known as the \textit{Fourier shift property}. A Fourier transform can also be defined on other groups, resulting in maps equivariant to more general transformations in the input, such as 2D and 3D rotations \cite{rudin1964fourier}. This fact has been capitalized upon in recent years with a proliferation of recent papers that generalize standard translation-equivariant convolutional neural networks (CNNs) to other groups\textemdash a line of work known as Geometric Deep Learning \cite{bronstein2021geometric}. [which has demonstrated great promise]

% Importantly, the Fourier/convolution operation is \textit{unique} as a linear equivariant map. All other linear equivariant maps are provably equivalent, up to [perms etc]. This means that the Fourier transform is a universal solution to the problem of equivariance in a single neural network layer. This fact may explain the pervasiveness of learned Fourier-based features in 


% In this work, we argue that the 

% Indeed, the \textit{only} linear equivariant map for a given group is a Fourier transform (equivalently, a convolution). That is, the Fourier transform is a unique solution to the problem of equivariance in a single neural network layer. [Strong mathematical basis for this work.]

% In this work, we ask whether there are similar mathematical guarantees for \textit{invariant} neural network layers.

% \textemdash in the form of its spatial convolutional dual\textemdash b

 % Most are familiar with the Fourier transform as a method for frequency decomposition. Its group theoretic foundation is less well known.

% \textit{equivariance} to the group of translation\textemdash a fact that is exploited in Geometric Deep Learning to construct equivariant CNNs for groups of transformations that go beyond translation. 

% In recent years, a line of work has emerged that makes use of the connection between the Fourier transform and its mathematical foundations in group representation theory. This has permitted the generalization of conventional translation-equivariant convolutional neural networks (CNNs) to other groups \cite{}. 

% Fourier analysis has a long history in signal processing. From the perspective of he Fourier domain offers many desi

% In this paper, we present a novel result

% An intelligent agent must form representations of the world that are \textit{general}\textemdash robust to the many variations in sensory data that the natural world imparts. 

% A fundamental problem of intelligence is to form representations of the world that separate 

% A core property of 

% Pitts and McCullough\textemdash widely regarded as the inventors of the first artificial neural network \cite{mcculloch1943logical}\textemdash referred to such form-selective representations as \textit{universals} \cite{pitts1947we}.
% In this paper, we present a novel theorem rooted in invariant theory and algebraic geometry that proves the uniqueness of higher-order spectral invariants as solutions to the problem of invariant representation learning. 

% This finding provides support for the use of neural network architectures that restrict the solution class to the set of higher-order spectral invariants \cite{sanborn2023bispectral}.

% Possible results:
%  - Spectral Uniqueness
%  - Power Spectral Model (convex?)
%  - Uniqueness of the bispectrum on homogeneous x invariant? (Nina)
%  - Empirical results showing training under noise
%  - Empirical results showing gabors for local translation?


% The ability to form \textit{invariant representations} is central to intelligence. Invariance plays a fundamental role in many deep learning algorithms. Despite this, few papers in the field have made use of the rich set of mathematical tools provided by invariant theory and algebraic geometry \cite{sturmfels2008algorithms}. In this paper, we use techniques from algebraic geometry and theorems fundamental to invariant theory to provide novel guarantees regarding neural network solutions to invariant representation learning. 

% a large body of relevant results in pure mathematics from the fields of invariant theory and algebraic geometry, there has been surprisingly little crossover from these fields into machine learning. In the context of deep learning, invariance is commonly approached in an informal way. 



% derive a novel principle for neural coding.


% This paper tackles the following question: \textit{Is there a mathematically universal solution to the problem of invariant representation learning?}

% The ability to \textit{generalize} is core to intelligence. At the heart of the problem of generalization is \textit{invariance}. In order to generalize from one context to another, one must be able to pull out the features that are constant despite myriad surface-level changes. 

% A fundamental problem of intelligence is to form representations of the world that are invariant to transformations that are task-irrelevant. 


%%%%%%%%%%%%%%%%%
% VERSION 3 WIP % 
%%%%%%%%%%%%%%%%%





% [CJH refs and pointing to parallel stories for uniqueness:

% Original motivation from neuroscience: compressive channel coding using compressed sensing methodology \cite{isely2010deciphering}

% Uniqueness sparse coding zero error: \cite{hillar2015can}

% Uniqueness, Robust (noisy) case):  \cite{garfinkle2019uniqueness}]


\section{Related Work}\label{sec:specrelwork}


\subsection{Emergence of Fourier Features}
\begin{itemize}
    \item Sparse coding etc
    \item Fourier features in networks learning arithmetic
    \item Possibly grid cells
    \item Polar predictor
    \item Temporal coherence
    \item Bispectral networks
    \item Gabors in deep networks (Chris Olah interpretability work)
\end{itemize}

\subsection{Invariant Machine Learning}
Invariance to symmetries is a natural bias for learning systems that has been extensively considered in the literature. It can be achieved by self-supervision or as an emergent by-product of downstream learning tasks.  ...[Invariant theory, Noether's theorem for symplectic invariants] 

Inferring the symmetries of data is a statistical problem known as \textbf{symmetry discovery}. Mathematically, the goal is recovering the group structure in some form of the unknown symmetries of a dataset. The majority of the literature focuses on discovering a group of linear transformations fixing a dataset in the Euclidean space. By assuming that the group is a differentiable manifold (i.e., a Lie group), the problem can be recast via the matrix exponential as learning linearly-independent generators of the tangent space (i.e., the Lie algebra). The line of works \cite{rao1998learning, miao2007learning} proposes to directly fit the generators, which has been subsequently extended in \cite{sohl2010unsupervised} by  introducing a smoothing regularization. The same principle has been alternatively implemented in \cite{desai2022symmetry, yang2023generative} via a fitting procedure involving an adversarial discriminator. 

\subsection{Complex-Valued Machine Learning}
Since harmonic analysis relies crucially on complex numbers, in this work we focus on networks with complex weights. This fits into the line of research initiated by \cite{clarke1990generalization} aimed at exploring complex-valued machine learning models and extending standard constructions to the complex case \cite{trabelsi2017deep}. Such models have seen applications, for example, in audio processing \cite{hirose2012generalization}, radar data \cite{yao2019complex}, and cryptography \cite{dong2019neural}. We refer the reader to  \cite{bassey2021survey} for a survey. In particular, recent work has observed the emergence of 



==> sections/2-background.tex <==
% \input{sections/intro_invariant_theory}

\section{Mathematical Background}
\label{sec:background}


We begin by introducing the fundamental concepts from harmonic analysis and group theory used in this paper. For a complete treatment, we refer the reader to \cite{folland2016course}. 

% In this section we outline the principles of group theory together with harmonic analysis over groups. For a complete treatment we refer to \cite{folland2016course}. 

\subsection{Groups and Actions}
We start by recalling the notion of a group. Intuitively, a group is an algebraic object whose elements represent abstract symmetries. The latter can be composed and inverted, leading to the following definition.  

\begin{defn}\label{groupdef}
A group is a set $G$ equipped with a \emph{composition map} $G \times G \rightarrow G$ denoted by $(g,h) \mapsto gh$, an \emph{inversion map} $G \rightarrow G$ denoted by $g \mapsto g^{-1}$, and a distinguished \emph{identity element} $1 \in G$ such that for all $g, h, k \in G$:
\begin{center}
\begin{tabular}{ccc}
\emph{Associativity} &   \emph{Inversion} & \emph{Identity}  \\
 $g(hk) = (gh)k$ & \hspace{.2cm} $g^{-1}g = g g^{-1} = 1$  \hspace{.2cm} & $g1 = 1g = g$ 
\end{tabular}
\end{center}
A map $\lambda: \ G \rightarrow G'$ between groups is called \emph{homomorphism} if $\lambda(gh) = \lambda(g) \lambda(h)$ for all $g,h \in G$.  
\end{defn}
Examples of groups include the permutations of a set and the general linear group $\textnormal{GL}(n)$ of $n \times n$ invertible real matrices, both equipped with usual composition and inversion of functions. Groups satisfying $gh = hg$ for all $g,h \in G$ are said to be \emph{commutative} or, alternatively, \emph{Abelian}. 

The idea of a space $\mathcal{X}$ having $G$ as a group of symmetries is abstracted by the notion of group \emph{action}. 
\begin{defn}\label{actiondef}
An action by a group $G$ on a set $\mathcal{X}$ is a map $G \times \mathcal{X} \rightarrow \mathcal{X}$ denoted by $(g,x) \mapsto g \cdot x$, satisfying for all $g,h \in G, \ x \in \mathcal{X}$: 
\begin{center}
\begin{tabular}{ccc}
\emph{Associativity} & \hspace{1cm} & \emph{Identity} \\
$g\cdot (h \cdot x) = (gh) \cdot x$ & \hspace{1cm} &  $1 \cdot x = x$
 \end{tabular}
  \end{center}
A map $\varphi \colon \ \mathcal{X} \rightarrow \mathcal{Z}$ between sets acted upon by $G$ is called \emph{equivariant} if $\varphi(g \cdot x) = g \cdot \varphi(x)$ for all $g \in G, x\in \mathcal{X}$. It is called \emph{invariant} if moreover $G$ acts trivially on $\mathcal{Z}$ or, explicitly, if  $\varphi(g \cdot x) = \varphi(x)$. 
\end{defn}
In general, the following actions can be defined for arbitrary groups: $G$ acts on any set \emph{trivially} by $g \cdot x = x$, and $G$ acts on itself seen as a set via (left) \emph{multiplication} by  $g \cdot h = gh$. A further example of group action is $\textnormal{GL}(n)$ acting on $\mathbb{R}^n$ by matrix multiplication. 


\subsection{Harmonic Analysis on Groups}
We now review harmonic analysis of signals over groups. This generalizes the usual harmonic analysis via the Fourier transform. We focus on the finite groups for simplicity, which are sufficient for practical applications. This avoids technicalities such as integrability conditions and continuity issues arising for infinite groups. Moreover, for the following sections we assume that $G$ is Abelian, which greatly simplifies harmonic analysis. We discuss the non-Abelian case in Section \ref{sec:nonabelian}. 

Let $G$ be a finite Abelian group. Denote by $\free{G} = \mathbb{C}^G$ the free complex vector space generated by $G$. Intuitively, an element $x = (x_g)_{g \in G} \in \free{G}$ represents a complex-valued signal over $G$. The space $\free{G}$ is endowed with the \emph{convolution} product
\begin{equation}
(x \star y)_g = \sum_{h \in G}x_h y_{h^{-1}g}.
\end{equation}
 and is acted upon by $G$ via $g \cdot x = \delta_g \star x = (x_{g^{-1}h})_{h \in G}$, where $\delta_g$ is the canonical basis vector. 
\begin{defn}
The \emph{dual} $G^\vee$ of $G$ is the set of homomorphisms $\lambda: \ G \rightarrow \textnormal{U}(1)$, where $\textnormal{U}(1) \subseteq \mathbb{C}$ is the group of unitary complex numbers equipped with multiplication. It is itself a group when equipped with the pointwise composition $(\lambda \mu)(g) = \lambda(g) \mu(g)$.
\end{defn}
A homomorphism $\lambda \in G^\vee$ intuitively represents a \emph{harmonic} over $G$, generalizing the familiar notion from signal processing. If we endow $\free{G}$ with the normalized scalar product $\langle x, y \rangle = \frac{1}{|G|} \sum_{g \in G} \overline{x_g} y_g$ then $G^\vee \subseteq \free{G}$ forms an orthonormal basis. The linear base-change is, by definition, the Fourier transform over $G$: 
\begin{defn}\label{transform}
The \emph{Fourier transform} is the map $\free{G} \rightarrow \free{G^\vee}$, $x \mapsto \hat{x}$, defined for $\lambda \in G^\vee$ as: 
\begin{equation}\label{fourier}
\hat{x}_\lambda = \langle \lambda, x \rangle.  
\end{equation}
\end{defn}
The Fourier transform is an isometry and exchanges the convolution product $\star$ over $\free{G}$ with the Hadamard product $\odot$ over $\free{G^\vee}$. Definition \ref{transform} generalizes the usual (discrete) Fourier transform in the following sense. For an integer $d>0$, consider the group $G=\mathbb{Z}/d\mathbb{Z}$ is of integers modulo $d$ equipped with addition as composition. The dual $G^\vee$ consists of homomorphisms of the form 
\begin{equation}
\mathbb{Z} / d\mathbb{Z} \ni g \mapsto e^{2 \pi \sqrt{-1} g k/d}
\end{equation}
for $k \in \{0, \cdots, d-1 \}$. Equation \ref{fourier} recovers then the familiar definition of the Fourier transform.  



\subsection{Spectral Invariants}
We now focus on the \emph{invariants} over $\free{G}$ i.e., maps $\free{G} \rightarrow \mathbb{C}$ which are invariant w.r.t. the action by $G$. To this end, we recall the following polynomial invariants.  

\begin{defn}\label{specdef}
Fix $n>0$ and $\underline{\lambda} = (\lambda_1, \cdots, \lambda_{n}) \in (G^\vee)^{n}$. The \emph{spectrum of order} $n$ associated to $\underline{\lambda}$ is defined for $x \in \free{G}$ as: 
\begin{equation}\label{spectralformula}
\beta_{\underline{\lambda}}(x) =  \hat{x}_{\lambda_1} \cdots \hat{x}_{\lambda_n}   \overline{\hat{x}}_{\lambda_1 \cdots \lambda_n}
\end{equation}
\end{defn}
The spectra of order $n$ are invariant polynomials of degree $n+1$ containing one conjugate variable. The presence of the latter is necessary for invariance. For $n=1,2$ they are alternatively referred to as \emph{power spectra} and \emph{bispectra} respectively. Note that the power spectra reduce simply to $\beta_{\lambda}(x) = |  \hat{x}_{\lambda}  |^2 $ for $\lambda \in G^\vee$. A remarkable aspect of spectra of order at least $2$ is the fact that they jointly determine real (generic) elements of $\free{G}$ up to the action by $G$ -- a property known as \emph{completeness}. 

\begin{prop}\label{complete}
Fix $n \geq 2$. Suppose $x,y \in \mathbb{R}^G \subseteq \free{G}$ are such that $\langle x, \lambda \rangle$, $\langle y, \lambda \rangle \not = 0$ for all $\lambda \in G^\vee$. If $\beta_{\underline{\lambda}}(x) = \beta_{\underline{\lambda}}(y)$ for all $\underline{\lambda} \in (G^\vee)^{n}$ then $x = g \cdot y$ for some $g \in G$. 
\end{prop}
\begin{proof}
By setting $\underline{\lambda} = (1, \cdots ,1)$ we see that $\langle 1,x \rangle^{n+1} = \langle  1, y \rangle^{n+1}\in \mathbb{R} \setminus \{0 \}$ and therefore $ | \langle 1, y\rangle |  =  | \langle 1,y \rangle | $. For $\lambda \in G^\vee$, by setting $\underline{\lambda} = (\lambda, \overline{\lambda}, 1, \cdots, 1)$ we see that $ \langle \lambda,x \rangle  \langle \overline{\lambda}, x \rangle  \langle 1,x \rangle^{n-1} = | \langle \lambda,x \rangle |^2  \langle 1,x \rangle^{n-1}  =  | \langle \lambda,y \rangle |^2  \langle 1,y \rangle^{n-1}    $ and therefore $| \langle \lambda,x \rangle | = | \langle \lambda,y \rangle |$. Note that here we relied on the fact that $x$ and $y$ are real. This implies that the following map $\eta: \ G^\vee \rightarrow \mathbb{C}$ takes values in $\textnormal{U}(1) \subseteq \mathbb{C}$: 
\begin{equation}
\eta(\lambda) = \pm \frac{\langle \lambda, x \rangle }{ \langle \lambda,y \rangle }. 
\end{equation}
Here the sign is determined as $\pm = \frac{\langle 1,x \rangle^{n}}{\langle 1, y \rangle^{n}}$. Note that $\eta(1) = 1$ since $ \langle 1, y\rangle^{n+1}  =  \langle 1,y \rangle^{n+1} $. By setting $\underline{\lambda} = (\lambda, \mu, \overline{\lambda \mu}, 1, \cdots  , 1)$ we see that $\eta(\lambda) \eta(\mu) = \eta(\overline{\lambda \mu})$ for all $\lambda, \mu \in G^\vee$ and therefore $\eta \in (G^\vee)^\vee$. Since the Fourier transform sends $G^\vee \subseteq \free{G}$ to $(G^\vee)^\vee \subseteq \free{G^\vee}$, there exists $g\in G$ such that $\eta(\lambda) = \overline{\lambda(g)}$. This means that $ \langle \lambda , x\rangle  =  \overline{\lambda(g)} \langle \lambda ,y \rangle $, which implies $x = g \cdot y$ by the equivariance properties of the Fourier transform.  
\end{proof}




\subsection{Bispectral Networks}
Inspired by Propositions \ref{complete}, a machine learning model under the name \emph{Bipectral Network} has been recently introduced in \cite{sanborn2023bispectral}. The overall idea is to train a model to approximate the bispectrum for an \emph{unknown group} $G$. Given an integer $d > 0$ representing the cardinality of $G$, the Bispectral Network is defined as the collection of parametric maps $\omega:  \ \mathbb{C}^d \rightarrow \mathbb{C}^{d \times d}$ given by: 
\begin{equation}\label{bispecnet}
\omega_{i,j}(x) = W_ix \ W_j x  \ \overline{W_i \odot W_j \ x}
\end{equation}
where $W$ is a $d \times d$ complex matrix. The latter is the parameter to be optimized and is meant to represent the (unknown) Fourier transform of $G$. The expression for $\omega_{i,j}$ mimics Equation \ref{spectralformula} for $n=2$. The Bispectral Network optimizes then an objective encouraging $\omega$ to be invariant and $W$ to be unitary. Namely, given a finite dataset $\mathcal{D}$ of pairs $(x,y) \in \mathbb{C}^d$ where $x = g \cdot y$ for an unknown $g \in G$, the objective is:
\begin{equation}
\mathcal{L}(W) = \sum_{(x,y) \in \mathcal{D}} \|\omega(x) - \omega(y)\|^2 + \eta \ \| x - W^\dagger W x \|^2  
\end{equation}
7where $^\dagger$ denotes the transpose conjugate and $\eta > 0$ is a hyper-parameter. Therefore, Bispectral Networks implement a form of \emph{contrastive learning} via a cubical polynomial in the form of the bispectrum.   




% We now focus on the \emph{invariants} over $\free{G}$ i.e., maps $\free{G} \rightarrow \mathbb{C}$ which are invariant w.r.t. the action by $G$. To this end, we recall the following polynomial invariants.  

% \begin{defn}\label{specdef}
% Fix $n>0$ and let $\underline{\lambda} = (\lambda_1, \cdots, \lambda_{n+1}) \in (G^\vee)^{n+1}$ be such that $\prod_{1 \leq i \leq n+1} \lambda_i = 1$. The \emph{spectrum of order} $n$ associated to $\underline{\lambda}$ is defined for $x \in \free{G}$ as: 
% \begin{equation}
% \beta_{\underline{\lambda}}(x) = \prod_{1 \leq i \leq n+1} \hat{x}_{\lambda_i}
% \end{equation}
% \end{defn}
% The spectra of order $n$ are invariant polynomials of degree $n+1$. For $n=1,2$ they are alternatively referred to as \emph{power spectra} and \emph{bispectra} respectively. Now, it turns out that spectra generate all the polynomial invariants of $\free{G}$.
% \begin{prop}\label{mainth}
% The space of polynomial invariants of degree $n+1$ over $\free{G}$ is generated as a complex vector space by the spectra of order $n$.
% \end{prop}
% \begin{proof}
%  This follows from interpreting the invariance condition via the Fourier transform. Namely, given $\underline{\lambda} \in (G^\vee)^{n+1}$ consider the monomial over $\free{G^\vee}$ defined by $\prod_{1 \leq i \leq n+1}\hat{x}_{\lambda_i}$. Since $g \cdot \hat{x} = (\overline{\lambda(g)} \hat{x}_\lambda)_{\lambda \in G^\vee}$, the monomial is invariant if and only if $\prod_{1 \leq i \leq n+1} \lambda_i(g) = 1$ for all $g \in G$, from which the claim follows.  
% \end{proof}

% A remarkable fact about spectra of order at least $2$ is the fact that they jointly determine real (generic) elements of $\free{G}$ up to the action by $G$ -- a property known as \emph{completeness}. 

% \begin{prop}\label{complete}
% Fix $n \geq 2$. Suppose $x,y \in \mathbb{R}^G \subseteq \free{G}$ are such that $\langle x, \lambda \rangle$, $\langle y, \lambda \rangle \not = 0$ for all $\lambda \in G^\vee$. If $\beta_{\underline{\lambda}}(x) = \beta_{\underline{\lambda}}(y)$ for all $\underline{\lambda} \in (G^\vee)^{n+1}$ such that $\prod_{1 \leq i \leq n+1}\lambda_i = 1$ then $x = g \cdot y$ for some $g \in G$. 
% \end{prop}
% \begin{proof}
% By setting $\underline{\lambda} = (1, \cdots ,1)$ we see that $\langle 1,x \rangle^{n+1} = \langle  1, y \rangle^{n+1}\in \mathbb{R} \setminus \{0 \}$ and therefore $ | \langle 1, y\rangle |  =  | \langle 1,y \rangle | $. For $\lambda \in G^\vee$, by setting $\underline{\lambda} = (\lambda, \overline{\lambda}, 1, \cdots, 1)$ we see that $ \langle \lambda,x \rangle  \langle \overline{\lambda}, x \rangle  \langle 1,x \rangle^{n-1} = | \langle \lambda,x \rangle |^2  \langle 1,x \rangle^{n-1}  =  | \langle \lambda,y \rangle |^2  \langle 1,y \rangle^{n-1}    $ and therefore $| \langle \lambda,x \rangle | = | \langle \lambda,y \rangle |$. Note that here we relied on the fact that $x$ and $y$ are real. This implies that the following map $\eta: \ G^\vee \rightarrow \mathbb{C}$ takes values in $\textnormal{U}(1) \subseteq \mathbb{C}$: 
% \begin{equation}
% \eta(\lambda) = \pm \frac{\langle \lambda, x \rangle }{ \langle \lambda,y \rangle }. 
% \end{equation}
% Here the sign is determined as $\pm = \frac{\langle 1,x \rangle^{n}}{\langle 1, y \rangle^{n}}$. Note that $\eta(1) = 1$ since $ \langle 1, y\rangle^{n+1}  =  \langle 1,y \rangle^{n+1} $. By setting $\underline{\lambda} = (\lambda, \mu, \overline{\lambda \mu}, 1, \cdots  , 1)$ we see that $\eta(\lambda) \eta(\mu) = \eta(\overline{\lambda \mu})$ for all $\lambda, \mu \in G^\vee$ and therefore $\eta \in (G^\vee)^\vee$. Since the Fourier transform sends $G^\vee \subseteq \free{G}$ to $(G^\vee)^\vee \subseteq \free{G^\vee}$, there exists $g\in G$ such that $\eta(\lambda) = \overline{\lambda(g)}$. This means that $ \langle \lambda , x\rangle  =  \overline{\lambda(g)} \langle \lambda ,y \rangle $, which implies $x = g \cdot y$ by the properties of the Fourier transform.  
% \end{proof}

% \subsection{Bispectral Networks}
% Inspired by Propositions \ref{mainth} and \ref{complete}, a machine learning model under the name \emph{Bipectral Network} has been recently introduced in \cite{sanborn2022bispectral}. The overall idea is to train a model to approximate the bispectrum for an \emph{unknown group} $G$. Given an integer $d > 0$ representing the cardinality of $G$, the Bispectral Network is defined as the collection of parametric maps $\omega:  \ \mathbb{C}^d \rightarrow \mathbb{C}^{d^2}$ given by: 
% \begin{equation}\label{bispecnet}
% \omega_{i,j}(x) = W_ix \ W_j x  \ \overline{W_i \odot W_j}x
% \end{equation}
% where $W$ is a $d \times d$ complex matrix. The latter is the parameter to be optimized and is meant to represent the (unknown) Fourier transform of $G$. The factor of Equation \ref{bispecnet} involving the Hadamard product is designed to impose the condition on $\underline{\lambda}$ from Definition \ref{specdef}. The Bispectral Network optimizes then an objective encouraging $\omega$ to be invariant and $W$ to be unitary. Namely, given a finite dataset $\mathcal{D}$ of pairs $(x,y) \in \mathbb{C}^d$ where $x = g \cdot y$ for an unknown $g \in G$, the objective is:
% \begin{equation}
% \mathcal{L}(W) = \sum_{(x,y) \in \mathcal{D}} \|\omega(x) - \omega(y)\|^2 + \eta \ \| x - W^\dagger W x \|^2  
% \end{equation}
% 7where $^\dagger$ denotes the transpose conjugate and $\eta > 0$ is a hyper-parameter. Therefore, Bispectral Networks implement a form of \emph{contrastive learning} via a cubical polynomial in the form of the bispectrum.   

% {\color{red}---------------- Revised Until Here ----------------} \\

% \subsection{CNNs}
% % Lossy invariance objective

% \subsection{Transformers}
% % Could they be bispectral networks in disguise?

% \subsection{Sparse Coding \& ICA}
% % Note that there is no invariance objective for sparse coding and ICA
% % Include Pierre-Etienne's paper and make a note about the equivariance objective? Fourier guaranteed as convolution is the only linear equivariant map

% By setting $\underline{\lambda} = (1,1,1)$ we see that $\langle 1,x \rangle^3 = \langle  1, y \rangle^3 \in \mathbb{R} \setminus \{0 \}$ and therefore $ \langle 1, y\rangle  =  \langle 1,y \rangle $. For $\lambda \in G^\vee$, by setting $\underline{\lambda} = (\lambda, \overline{\lambda}, 1)$ we see that $ \langle \lambda,x \rangle  \langle \overline{\lambda}, x \rangle  \langle 1,x \rangle = | \langle \lambda,x \rangle |^2  \langle 1,x \rangle  =  | \langle \lambda,y \rangle |^2  \langle 1,y \rangle    $ and therefore $| \langle \lambda,x \rangle | = | \langle \lambda,y \rangle |$. Note that here we relied on the fact that $x$ and $y$ are real. This implies that the map $\eta: \ G^\vee \rightarrow \mathbb{C}$ defined as 
% \begin{equation}
% \eta(\lambda) = \frac{\langle \lambda, x \rangle }{ \langle \lambda,y \rangle } 
% \end{equation}
% takes values in $\textnormal{U}(1) \subseteq \mathbb{C}$. Note that $\eta(1) = 1$ since $ \langle 1, y\rangle  =  \langle 1,y \rangle $. Invariance of the bispectrum implies moreover that $\eta(\lambda) \eta(\mu) = \eta(\overline{\lambda} \overline{\mu})$ for all $\lambda, \mu \in G^\vee$ and therefore $\eta \in (G^\vee)^\vee$. Since the Fourier transform sends $G^\vee \subseteq \free{G}$ to $(G^\vee)^\vee \subseteq \free{G^\vee}$, there exists $g\in G$ such that $\eta(\lambda) = \overline{\lambda(g)}$. This means that $ \langle \lambda , x\rangle  =  \overline{\lambda(g)} \langle \lambda ,y \rangle $, which implies $x = g \cdot y$ by the properties of the Fourier transform.   
% \end{proof}


==> sections/2-background_new.tex <==
% \input{sections/intro_invariant_theory}

\section{Mathematical Background}
\label{sec:background}

We begin by introducing the fundamental concepts from harmonic analysis and group theory used in this paper. For a complete treatment, we refer the reader to \cite{folland2016course}. 
%We provide a one-page introduction to these mathematical foundations in Appendix \ref{appendix:math}.


\subsection{Groups and Actions}
\label{appendix:math}


% We start by recalling the notion of a group. Intuitively, a group is an algebraic object whose elements represent abstract symmetries. The latter can be composed and inverted, leading to the following definition.  

A \textit{group} is an algebraic object whose elements represent abstract symmetries, which can be composed and inverted.

% \textbf{Groups and Actions} 
\begin{defn}\label{groupdef}
A group is a set $G$ equipped with a \emph{composition map} $G \times G \rightarrow G$ denoted by $(g,h) \mapsto gh$, an \emph{inversion map} $G \rightarrow G$ denoted by $g \mapsto g^{-1}$, and a distinguished \emph{identity element} $1 \in G$ such that for all $g, h, k \in G$:
\begin{center}
\begin{tabular}{ccc}
\emph{Associativity} &   \emph{Inversion} & \emph{Identity}  \\
 $g(hk) = (gh)k$ & \hspace{.2cm} $g^{-1}g = g g^{-1} = 1$  \hspace{.2cm} & $g1 = 1g = g$    
\end{tabular}
\end{center}
A map $\rho: \ G \rightarrow G'$ between groups is called a \emph{homomorphism} if $\rho(gh) = \rho(g) \rho(h)$ for all $g,h \in G$.  
\end{defn}
Examples of groups include the permutations of a set and the general linear group $\textnormal{GL}(V)$ of invertible operators over a vector space $V$, both equipped with the usual composition and inversion of functions. A further example that will be relevant in this work is the \emph{unitary} group $\textnormal{U}(V) \subseteq \textnormal{GL}(V)$ associated to a Hilbert space $V$, consisting of operators $U$ satisfying $UU^{\dagger} = I$, where $\dagger$ denotes the conjugate transpose and $I$ is the identity matrix. Groups satisfying $gh = hg$ for all $g,h \in G$ are deemed \emph{commutative}.

The idea of a space $\mathcal{X}$ having $G$ as a group of symmetries is abstracted by the notion of group \emph{action}. 
\begin{defn}\label{actiondef}
An action by a group $G$ on a set $\mathcal{X}$ is a map $G \times \mathcal{X} \rightarrow \mathcal{X}$ denoted by $(g,x) \mapsto g \cdot x$, satisfying for all $g,h \in G, \ x \in \mathcal{X}$: 
\begin{center}
\begin{tabular}{ccc}
\emph{Associativity} & \hspace{1cm} & \emph{Identity} \\
$g\cdot (h \cdot x) = (gh) \cdot x$ & \hspace{1cm} &  $1 \cdot x = x$
 \end{tabular}
  \end{center}


A map $\varphi \colon \ \mathcal{X} \rightarrow \mathcal{Z}$ between sets acted upon by $G$ is called \emph{equivariant} if $\varphi(g \cdot x) = g \cdot \varphi(x)$ for all $g \in G, x\in \mathcal{X}$. It is called \emph{invariant} if moreover $G$ acts trivially on $\mathcal{Z}$ or, explicitly, if  $\varphi(g \cdot x) = \varphi(x)$. 
\end{defn}
In general, the following actions can be defined for arbitrary groups: $G$ acts on any set \emph{trivially} by $g \cdot x = x$, and $G$ acts on itself seen as a set via (left) \emph{multiplication} by  $g \cdot h = gh$. Further examples are $\textnormal{GL}(V)$ and $\textnormal{U}(V)$ acting on $V$ by evaluating operators. 



% In this section we outline the principles of group theory together with harmonic analysis over groups. For a complete treatment we refer to \cite{folland2016course}. 




\subsection{Harmonic Analysis on Groups}

% We first review harmonic analysis of signals over groups. 
Harmonic analysis on groups \cite{rudin1964fourier} generalizes standard harmonic analysis. We focus here on finite groups for simplicity, which are sufficient for practical applications. This avoids technicalities such as integrability conditions and continuity issues arising for infinite groups. We start by considering commutative groups and cover non-commutative ones in Section \ref{sec:nonabelian}.

% Moreover, for the following sections we assume that $G$ is commutative, which greatly simplifies harmonic analysis. We discuss the non-commutative case in Section \ref{sec:nonabelian}. 

Let $G$ be a finite commutative group of order $|G|$. Denote by $\free{G} = \mathbb{C}^G$ the free complex vector space generated by $G$. Intuitively, an element $x = (x_g)_{g \in G} \in \free{G}$ represents a complex-valued signal over $G$. The space $\free{G}$ is endowed with the \emph{convolution} product,
\begin{equation}\label{eq:convol}
(x \star y)_g = \sum_{h \in G}x_h y_{h^{-1}g},
\end{equation}
 and is acted upon by $G$ via $g \cdot x = \delta_g \star x = (x_{g^{-1}h})_{h \in G}$, where $\delta_g$ is the canonical basis vector. 
\begin{defn}
The \emph{dual} $G^\vee$ of $G$ is the set of homomorphisms $\rho: \ G \rightarrow \textnormal{U}(1)$, where $\textnormal{U}(1) \subseteq \mathbb{C}$ is the group of unitary complex numbers equipped with multiplication. It is itself a group when equipped with pointwise composition $(\rho \mu)(g) = \rho(g) \mu(g)$.
\end{defn}
A homomorphism $\rho \in G^\vee$ intuitively represents a \emph{harmonic} over $G$, generalizing the familiar notion from signal processing. If we endow $\free{G}$ with the canonical scalar product $\langle x, y \rangle = \sum_{g \in G} \overline{x_g} y_g$, then $G^\vee \subseteq \free{G}$ forms an orthogonal basis with all the norms equal to $|G|$. The linear base-change is, by definition, the Fourier transform over $\free{G}$: 
\begin{defn}\label{transform}
The \emph{Fourier transform} is the map $\free{G} \rightarrow \free{G^\vee}$, $x \mapsto \hat{x}$, defined for $\rho \in G^\vee$ as: 
\begin{equation}\label{fourier}
\hat{x}_\rho = \langle \rho, x \rangle.  
\end{equation}
\end{defn}
The Fourier transform is a linear isometry or, equivalently, a unitary operator, up to a multiplicative constant of $|G|$. Moreover, it exchanges the convolution product $\star$ over $\free{G}$ with the Hadamard product $\odot$ over $\free{G^\vee}$. Definition \ref{transform} generalizes the usual discrete Fourier transform in the following sense. For an integer $d>0$, consider the cyclc group $C_d$ with $d$ elements. Concretely $G=\mathbb{Z}/d\mathbb{Z} \simeq C_d$ is the group of integers modulo $d$ equipped with addition as composition. The dual $G^\vee$ consists of homomorphisms of the form:
\begin{equation}
\mathbb{Z} / d\mathbb{Z} \ni g \mapsto e^{2 \pi \sqrt{-1} g k/d},
\end{equation}
for $k \in \{0, \cdots, d-1 \}$. Equation \ref{fourier} specializes then to the familiar definition of the Fourier transform.  



\subsection{Non-Commutative Harmonic Analysis}\label{sec:nonabelian}
So far, we have assumed that $G$ is commutative. In this section we briefly discuss the extension of Fourier theory to non-commutative groups. This however requires more elaborate theoretical tools, which we now introduce. To begin with, in order to perform harmonic analysis on general groups it is necessary to discuss unitary representations. The latter will play the role of \textit{matrix-valued harmonics}. 
\begin{defn} 
A \emph{unitary representation} of $G$ is an action by $G$ on a finite-dimensional Hilbert space $V$ via unitary operators or, in other words, a homomorphism $\rho_V: G \rightarrow \textnormal{U}(V)$. A unitary representation is said to be \emph{irreducible} if $V$ does not contain any non-trivial\footnote{The trivial sub-representations of $V$ are $0$ and $V$.} sub-representations. 
\end{defn}
We denote by $\irr{G}$ the set of all irreducible representations of $G$ up to isomorphism. Moreover, for a vector space $V$ we denote by $\textnormal{End}(V)$ the space of its linear operators.   

\begin{defn}
The \emph{Fourier transform} is the map $\free{G} \rightarrow \bigoplus_{\rho_V \in \irr{G}} \textnormal{End}(V)$, $x \mapsto \hat{x}$, defined for $\rho_V \in \irr{G}$ as: 
\begin{equation}\label{fouriernc}
\hat{x}_{\rho_V} = \sum_{g \in G}
\rho_V(g)^{\dagger} x_g \in \textnormal{End}(V).  
\end{equation}
\end{defn}
This generalizes Definition \ref{transform} since for a commutative group, $\rho_V$ is irreducible if, and only if, $\textnormal{dim}(V) = 1$. Analogously to the commutative setting, the Fourier transform exchanges the convolution product $\star$ with the point-wise operator composition, which we still denote by $\odot$. Moreover, the Fourier transform is a unitary operator up to a multiplicative constant of $|G|$ with respect to the normalized Hilbert-Schmidt scalar product on $\textnormal{End}(V)$, given by: 
\begin{equation}\label{eq:hilbsch}
\langle A, B \rangle = \textnormal{dim}(V) \  \textnormal{tr}(A^\dagger B).
\end{equation}

The norm associated to the Hilbert-Schmidt scalar product is the Frobenius norm. The relations between irreducible unitary representations coming from the unitarity of the Fourier transform are known as \emph{Schur orthogonality} relations. 



==> sections/3-theoretical-results.tex <==
\section{Theoretical Results}
\label{sec:theoretical-results}
We now present the primary theoretical contributions of this work. Concretely, we demonstrate that if certain parametric functions are invariant to a group then their weights must almost coincide with harmonics,  i.e. irreducible unitary group representations. We start by introducing general algebraic notions and principles, and then proceed to specialize them to machine learning scenarios. 

Let $G$ be a finite group, $\mathcal{H}$ be a set, and $V_1, \cdots, V_k$ be complex finite-dimensional Hilbert spaces. In what follows, we will consider the space
\begin{equation}
\mathcal{W} = \free{G} \otimes \bigoplus_i \textnormal{End}(V_i) \simeq \bigoplus_i \textnormal{End}(V_i)^{\oplus G}.
\end{equation}
$\mathcal{W}$ is a Hilbert space when endowed with the scalar product given by the product of the canonical scalar product over $\free{G}$ and the normalized Hilbert-Schmidt scalar products over $\textnormal{End}(V_i)$ (see Equation \ref{eq:hilbsch}). For $W \in \mathcal{W}$, we will denote each of its components as $W_i = (W_i(g))_g \in \textnormal{End}(V_i)^{\oplus G}$. Moreover, we will often interpret elements $W \in \mathcal{W}$ as linear maps $\free{G} \rightarrow \bigoplus_i \textnormal{End}(V_i)$ via $W(x) = \sum_{g \in G} W(g)x_g$ for $x \in \free{G}$, where $W(g) = (W_i(g))_i$. Note that $G$ acts on the left tensor factor of $\mathcal{W}$ while for each $i$, $\textnormal{U}(V_i)$ acts on the right tensor factor of $\free{G} \otimes \textnormal{End}(V_i)$ by composition of operators.     
\begin{defn}\label{def:symm}
We say that a map $\varphi \colon  \mathcal{W} \rightarrow \mathcal{H} $ has \emph{unitary symmetries} if for $W,W' \in \mathcal{W}$ of the same norm, $\varphi(W) = \varphi(W')$ implies that for each $i$ there exists a unitary operator $U_i \in \textnormal{U}(V_i)$ such that $W_i = U_i \cdot W_i'$.    
\end{defn}


In the context of machine learning, $\mathcal{H}$ will represent the \emph{hypothesis space}, consisting of functions the model can learn. On the other hand, $\varphi$ will represent the parametrization of such hypotheses, with its domain $\mathcal{W}$ being the space of weights. The component $\free{G}$ of $\mathcal{W}$ will be responsible for parametrizing the input space, while each component $\textnormal{End}(V_i)$ will represent a computational unit, i.e. a complex-valued \emph{neuron} in the language of neural networks. For commutative groups, we simply have $V_i = \mathbb{C} \simeq \textnormal{End}(V_i)$. In general, $\textnormal{End}(V_i)$ can be thought of as parametrizing matrix-valued signals, which, as mentioned in Section \ref{sec:overview}, are computed by neural units sometimes referred to as \emph{capsules} \cite{sabour2017dynamic}.  

The following is an abstract algebraic principle at the core of this work. 
\begin{thm}\label{prop:mainnew}
Suppose that $\varphi \colon \mathcal{W} \rightarrow \mathcal{H}$ has unitary symmetries and that for some $W \in \mathcal{W}$ the following holds:
\begin{itemize}
\item $\varphi(g \cdot W ) = \varphi(W)$ for all $g \in G$. 
\item $W_i$, seen as a linear map $\free{G} \rightarrow \textnormal{End}(V_i)$, is surjective for all $i$.
\end{itemize}
Then for every $i$ there exist $W_i' \in \textnormal{End}(V_i)$ and an irreducible unitary representation $\rho_i: \ G \rightarrow \textnormal{U}(V_i)$ such that for all $g \in G$,
\begin{equation}
W_i(g) = W_i' \rho_i(g)^\dagger. 
\end{equation}
\end{thm}
\begin{proof}
Since $\varphi$ has unitary symmetries and $\| g \cdot W \| = \| W \|$, it follows that for every $g \in G$ and every $i$ there exists $\rho_i(g) \in \textnormal{U}(V_i)$ such that
\begin{equation}\label{eq:generalw}
g \cdot W_i =  \rho_i(g) \cdot W_i . 
\end{equation}
In particular, by considering the component with index $1 \in G$ on both sides of Equation \ref{eq:generalw}, we see that $W_i(g^{-1}) = W_i(1) \ \rho_i(g)$. We wish to show that $\rho_i$ is a homomorphism. To this end, for all $g,h \in G$ it holds that
\begin{equation}\label{eq:generalproof}
 \rho_i(gh) \cdot W_i = (gh) \cdot W_i = g \cdot ( \rho_i(h) \cdot W_i ) = \rho_i(h) \cdot (g \cdot W_i)  = (\rho(g) \rho(h)) \cdot W_i.  
\end{equation}
By the surjectivity hypothesis, the set $\{W_i(g) \}_{g \in G}$ generates $\textnormal{End}(V_i)$ as a vector space. Therefore, Equation \ref{eq:generalproof} implies that $\rho_i(gh) = \rho_i(g) \rho_i(h)$, as desired. Lastly, note that $\rho_i$ is irreducible by the sujectivity assumption. Indeed, a nontrivial linear subspace of $V_i$ fixed by $\rho_i(g)$ for all $g$ would be sent by $W_i(g)$ into a fixed proper subspace due to Equation \ref{eq:generalw}. This contradicts the surjectivity of $W_i$. 
\end{proof}

Note that the surjectivity assumption implies the constraint $\sum_i \textnormal{dim}(V_i)^2 \leq |G|$. As a consequence of the result above, the full Fourier transform arises with an additional orthogonality assumption. 
\begin{cor}\label{mainpropnc}
Suppose that $\varphi \colon \mathcal{W} \rightarrow \mathcal{H}$ has unitary symmetries and that for some $W \in \mathcal{W}$ the following holds:
\begin{itemize}
\item $\varphi(g \cdot W ) = \varphi(W)$ for all $g \in G$. 
\item $W$ is unitary up to a multiplicative constant, i.e. $W^\dagger W = |G| I $. 
\end{itemize}
Then $W$ is the Fourier transform up to composing each of the components $W_i$ by an operator with Frobenius norm equal to $1$.
\end{cor} 
\begin{proof}
Note that the unitarity assumption above implies the surjectivity assumption from Theorem \ref{prop:mainnew}. Therefore, it follows that for every $i$, there exists an irreducible unitary representation $\rho_i : \ G \rightarrow \textnormal{U}(V_i)$ such that $W_i(g) = W_i(1) \ \rho_i(g)^\dagger$. We wish to show that if $i \not = j$ then $\rho_i$ and $\rho_j$ are non-isomorphic representations. If not, the orthogonality assumption implies that
\begin{align}   
0  = \sum_{g \in G}  \overline{W_i(g)} \otimes W_j(g)  & = \sum_{g \in G}  \left( \overline{W_i(1)} \otimes W_j(1)  \right) \left(  \rho_i(g)^{\top} \otimes \rho_j(g)^\dagger    \right) = \\
& =  |G| \  \overline{W_i(1)} \otimes W_j(1),
\end{align}
where $\top$ denotes the transpose and where the last identity follows from the Schur orthogonality relations. But then $W_i(1)$ or $ W_j(1)$ is vanishing, which contraddicts the unitarity assumption. 

Lastly, in order to compute the Frobenius norm of $W_i(1)$, note that 
\begin{equation}
|G| \ \| W_i(1) \|^2 = \sum_{g \in G} \| W_i(g) \ \rho_i(g) \|^2 = \sum_{g \in G} \| W_i(g) \|^2 = |G|,
\end{equation}
from which $\| W_i(1) \| = 1$ follows. 
\end{proof}
Again, the orthogonality assumption implies that $V_1, \cdots, V_k$ are the ambient Hilbert spaces of all the irreducible unitary representations of $G$ up to isomorphism, and in particular $\sum_i \textnormal{dim}(V_i)^2 = |G|$. 


We now wish to discuss the other crucial assumption of Theorem \ref{prop:mainnew} requiring that $\varphi(g \cdot W) = \varphi(W)$ for all $g \in G$, which is reminiscent of invariance. However, when $\mathcal{H}$ is a space of functions, we are typically interested in models that are invariant in the input variable rather than the weight variable. Therefore, we introduce the following condition, aimed at reconciling inputs and weights. To this end, suppose that $\mathcal{H}$ is a set of functions $\mathcal{X} \rightarrow \mathcal{Y}$, where $\mathcal{X}$ is a set acted upon by $G$ and $\mathcal{Y}$ is a set. We adhere to the notation $ \varphi(W, x) = \varphi(W)(x)$, $x \in \free{G}$, $W \in \mathcal{W}$, for simplicity.

\begin{defn}\label{defj:adj}
 We say that $\varphi$ satisfies the \emph{adjunction property} if
\begin{equation}
\varphi(W, g \cdot x) = \varphi(g^{-1} \cdot W, x) 
\end{equation}
for all $x\in \mathcal{X}, g \in G$. 
\end{defn}
The adjunction property implies that if $\varphi(W, x)$ is invariant in $x$, then $\varphi(g \cdot W, x) = \varphi(W, x)$ for all $x, g$, recovering the assumption of Theorem \ref{prop:mainnew}.

\begin{rmk}
As explained above, the tensor component $\free{G}$ of $\mathcal{W}$ typically represents the input space of a given machine learning model. One can consider the more general scenario when data consist of complex signals over a finite set $\mathcal{S}$ acted upon by $G$, therefore replacing $\free{G} = \mathbb{C}^G$ by $\mathbb{C}^\mathcal{S}$. This is the case, for example, for data consisting of images acted by the cyclic group via rotations, since the input space cannot be identified with signals over $G$. Assuming the action over $\mathcal{S}$ is \emph{free}, meaning that $g \cdot s = s$ implies $g=1$, $\mathcal{S}$ can be decomposed into copies of $G$ deemed \emph{orbits}. Specifically, there is an equivariant isomorphism $\mathcal{S} \simeq G \sqcup \cdots \sqcup G$, which in turn induces a linear isomorphism $\mathbb{C}^\mathcal{S} \simeq \free{G}^{\oplus p}$, where $p$ is the number of orbits. The results from this section can be extended to this scenario by applying all the arguments to the copies of $\free{G}$ separately, each of which will serve as a domain for its set of irreducible unitary representations. When the action is not free, it is necessary to take into account \emph{stabilizers}, i.e. $g \in G$ such that $g \cdot s = s$ for some $s \in \mathcal{S}$. Roughly speaking, we expect that the results from this section can be adapted to an extent, obtaining unitary representations `up to stabilizers'. However, the precise meaning of the latter has yet to be clarified, and goes beyond the scope of this work. 
\end{rmk}

\subsection{Examples}\label{sec:exmp}
In this section, we provide examples of machine learning models with unitary symmetries. As anticipated, in the context of machine learning $\mathcal{H}$ and $\mathcal{W}$ represent the hypothesis space and the parameter space, respectively. Indeed, in what follows $\mathcal{H}$ will consist of functions of the form $\free{G} \rightarrow \mathcal{Y}$ for some codomain $\mathcal{Y}$, and we will adhere to the notation from Definition \ref{defj:adj} accordingly. All the models considered in this section satisfy the adjunction property.

\subsubsection{Spectral Networks}\label{sec:specnet}
We start by considering \emph{Spectral Networks} -- a class of polynomial machine learning models that inspired this work\textemdash and to which our theory applies naturally. These models were introduced by \cite{sanborn2023bispectral} in cubic form based on the invariant theory of $\free{G}$ (see Section \ref{sec:specinv} in the Appendix for an overview of the latter). The overall idea behind Spectral Networks is to approximate the $n$-order polynomial invariants (deemed spectral invariants) of $\free{G}$ for an \emph{unknown} group $G$. Specifically, suppose that $V_1, \cdots, V_k$ are the ambient Hilbert spaces of the irreducible unitary representations of $G$. Given a multi-index $\underline{i} = (i_1, \cdots, i_n) \in \{1,  \cdots, k \}^n$, The Spectral Network of order $n$ is defined as the collection of parametric maps $\varphi_{\underline{i}}(W, \cdot):  \ \free{G}  \rightarrow \textnormal{End}(V_{i_1} \otimes \cdots \otimes V_{i_n})$: 
\begin{equation}\label{eq:ncspecnet}
\varphi_{\underline{i}}(W, x) =  W_{i_1} (x) \otimes \cdots \otimes W_{i_n}(x) \  \left( W_{i_1}^{\dagger} \odot   \cdots \odot W_{i_n}^{\dagger} \right) (\overline{x}),
\end{equation}
where $W=\oplus_iW_i \in \mathcal{W} = \free{G} \otimes  \oplus_i \textnormal{End}(V_i)$, $\odot$ denotes the $G$-wise tensor product of operators, and $\overline{x}$ denotes the component-wise conjugate of $x$. For a commutative $G$, since $V_i = \mathbb{C}$ for all $i$, the above expression reduces to:
\begin{equation}\label{bispecnet}
\varphi_{\underline{i}}(W, x) = W_{i_1}x  \cdots \ W_{i_n} x  \ \overline{W_{i_1} \odot \cdots \odot W_{i_n} \ x}.
\end{equation} 
 For $n=1$ Spectral Networks are deemed Power-Spectral Networks, and for a commutative $G$ they take the form $\varphi_i(W, x) = | W_i x |^2$. The latter can be simply interpreted as a linear model followed by an activation function. Even though the squared absolute value is uncommon as an activation function in machine learning, it has appeared in models of biological neural networks \cite{adelson1985spatiotemporal}. 

% On the same note, Spectral Networks for non-commutative groups can be defined as follows. Given a matrix $W \in \mathbb{C}^{d \times d}$, $d = |G|$, we think of it as a concatenation of $k$ tensors $W_i \in \mathbb{C}^{ d_i \times d_i \times d}$, where $d_1, \cdots, d_k$ are the dimensions of all the irreducible unitary representations of $G$. Given a multi-index $\underline{i} = (i_1, \cdots, i_n)$, we denote $d_{\underline{i}} = d_{i_1} \cdots d_{i_n}$. The \emph{Spectral Network} is then defined as the collection of parametric maps $\varphi_{\underline{i}}(W, \cdot):  \ \free{G} \simeq \mathbb{C}^d \rightarrow \mathbb{C}^{d_{\underline{i}} \times d_{\underline{i}}}$ given by: 
% \begin{equation}\label{eq:ncspecnet}
% \varphi_{\underline{i}}(W, x) =  ( W_{i_1} x )  \otimes \cdots \otimes (W_{i_n} x) \  \left( W_{i_1}^{\dagger} \overline{x} \ \otimes   \cdots \otimes W_{i_n}^{\dagger} \overline{x} \right).
% \end{equation}


For simplicity, we will consider only the Spectral Networks involving a single unitary representation; that is, we will focus on constant multi-indices $\underline{i} = (i, \cdots, i)$ in Equation \ref{eq:ncspecnet}. To this end, let $V$ be a finite-dimensional Hilbert space and $\mathcal{H}$ be the set of functions $\free{G} \rightarrow \textnormal{End}(V^{\otimes n})$ for some $n \in \mathbb{N}$. We set $\mathcal{W} = \free{G} \otimes \textnormal{End}(V)$. 
\begin{prop}\label{prop:specunitmain}
Consider the Spectral Network, given by:
\begin{equation}
\varphi(W, x) = W(x)^{\otimes n} \ W^{\dagger \odot n}(\overline{x}).
\end{equation}
Then $\varphi$ has unitary symmetries. 
\end{prop}
We refer to the Appendix for a proof. 


% We first focus on the commutative case, implying that $V = \mathbb{C}$ and therefore $W \in \free{G}$. Two examples of unitarily injective maps are: 
% \begin{itemize}
% \item \textit{Spectral Networks}: the model discussed in Section \ref{sec:specnet} obtained for a constant multi-index i.e.,
% \begin{equation}
% \varphi(W, x) = (Wx)^n \ \overline{W^{\odot n}x}
% \end{equation}
% for some $n > 0$. 
% \item \textit{McCulloch-Pitts Neurons}: a model of the form 
% \begin{equation}
%  \varphi(W,x) = \sigma(W x ),
% \end{equation}
% where $\sigma: \ \mathbb{C} \rightarrow \mathbb{C}$ is a map playing the role of an activation function. For $\sigma(z) = |z|^2$, this model reduces to a Spectral Network with $n=1$.    
% \end{itemize}

% Both the class of models above can be seen to satisfy the condition of unitarily injectivity, albeit with an assumption on $\sigma$.

\subsubsection{McCulloch-Pitts Neurons and Deep Networks}

% We now focus on another model common in neuroscience and machine learning, which we refer to as (complex) \emph{McCulloch-Pitts networks}. 

While Spectral Networks provide the most direct application of our theory, in this section we discuss the most common and fundamental neural network primitives in deep learning: the fully-connected McCulloch-Pitts neuron \cite{mcculloch1943logical} and the deep neural network. We consider models with complex coefficients and focus on commutative groups, i.e. all the Hilbert spaces $V_i$ from Definition \ref{def:symm} will be equal to $\mathbb{C}$. 

A McCulloch-Pitts neuron has the form $\varphi(W,x) = \sigma(W x )$, where $\sigma \colon \mathbb{C} \rightarrow \mathcal{Y}$ is a map playing the role of an activation function and $W \in \mathcal{W} = \free{G}$ is the weight vector. For $\sigma(z) = |z|^2$, the McCulloch-Pitts neuron reduces to a commutative Power-Spectral Network i.e., a Spectral Network with $n=1$.  The hypothesis space $\mathcal{H}$ consists of functions $\free{G} \rightarrow \mathcal{Y}$. 

\begin{prop}\label{lemm:mcculloch}
Consider a map $\sigma \colon \mathbb{C} \rightarrow \mathcal{Y}$ and let $\varphi(W,x) = \sigma(W x )$. Suppose that $0 \in \mathbb{C}$ is isolated in its fiber of $\sigma$, i.e. there exists an open subspace $O \subseteq \mathbb{C}$ such that $\sigma^{-1}(\sigma(0)) \cap O = \{ 0 \}$. Then $\varphi$ has unitary symmetries.
\end{prop}
We refer to the Appendix for a proof. The above assumption on $\sigma$ is satisfied by popular activations functions from neuroscience and machine learning, such as the sigmoid and the leaky Rectified Linear Unit (ReLU), applied after taking complex absolute value. 

% Next, we discuss the case of classical deep networks. We model the latter as $\varphi(W, x) = \chi(|W(x)|^2)$, where $W \in \mathcal{W} = \free{G} \otimes \mathbb{C}^k$ and $|\cdot|$ denotes the component-wise absolute value. Here, $k$ is the number of neurons in the first hidden layer of the network, while $\chi \colon \mathbb{R}_{\geq 0}^k \rightarrow \mathbb{R}$ is the head of the network, encompassing all the layers after the first one. Note that since typical neural networks are real-valued, we combine real and complex models. Namely, the first layer of $\varphi$ is complex, and its output is fed into the real head $\chi$ by taking squared absolute values. 

% % In what follows, we say that $\varphi(W,x)$ \emph{generically} has unitary hidden symmetries if Definition \ref{def:symm} holds for almost all $W \in \mathcal{W}$ i.e., if it holds in an open dense subspace of $\mathcal{W}$ (with the usual Euclidean topology). 
% Differently from Section \ref{sec:theoretical-results}, for the next result we will restrict $\mathcal{W}$ to the subspace of $\free{G} \otimes \mathbb{C}^k$ consisting of $W$ such that the components $W_i$ are orthonormal. This implies, in particular, the constraint $k \leq |G|$. Note that $\mathcal{W}$ is closed by the actions of $G$ and $\textnormal{U}(\mathbb{C})$. The orthonormality condition is anyway necessary in order to recover the full Fourier transform, as stated in Corollary \ref{mainpropnc}.  

% \begin{prop}\label{prop:deepnets}
% Suppose that there is an open subspace $O \subseteq \mathbb{R}_{\geq 0}^k$ containing $0$ where $\chi$ is affine with distinct non-vanishing coefficients i.e., $\chi(z) = \sum_i a_i z_i + b$ for $z \in O$ with $0 \not = a_i \not = a_j$ for $i \not = j$. Then $\varphi(W, x) = \chi(|W(x)|^2)$ has unitary symmetries. 
% \end{prop}  
% We refer to the Appendix for a proof. Since typical (real-valued) deep neural networks have piece-wise linear activations functions such as (leaky) ReLU, they define piece-wise affine maps and therefore are affine when restricted to appropriate open subspaces. Moreover, the hypothesis on the coefficients $a_i$ in Proposition \ref{prop:deepnets} is \emph{generic}, meaning that it defines an open dense subset of $(a_1, \cdots, a_k) \in \mathbb{R}^k$. 


Next, we discuss the case of classical deep networks. We model the latter as $\varphi(W, x) = \chi(\sigma(W(x)))$, where $W \in \mathcal{W} = \free{G} \otimes \mathbb{C}^k$ and $\sigma\colon \mathbb{C} \rightarrow \mathbb{R}$ represents the activation function, computed coordinate-wise on $\mathbb{C}^k$. Here, $k$ is the number of neurons in the first hidden layer of the network, while $\chi \colon \mathbb{R}^k \rightarrow \mathbb{R}$ is the head of the network, encompassing all the layers after the first one. Note that since typical neural networks are real-valued, we combine real and complex models. Namely, the first layer of $\varphi$ is complex, and its output is fed into the real head $\chi$ by applying the activation function. 

Differently from Section \ref{sec:theoretical-results}, for the next result we will restrict $\mathcal{W}$ to the subspace of $\free{G} \otimes \mathbb{C}^k$ consisting of $W$ such that the components $W_i$ are orthonormal. This implies, in particular, the constraint $k \leq |G|$. Note that $\mathcal{W}$ is closed by the actions of $G$ and $\textnormal{U}(\mathbb{C})$. The orthonormality condition is anyway necessary in order to recover the full Fourier transform, as stated in Corollary \ref{mainpropnc}.  

\begin{prop}\label{prop:deepnets}
Consider maps $\sigma \colon \mathbb{C} \rightarrow \mathbb{R}$, $\chi \colon \mathbb{R}^k \rightarrow \mathbb{R}$ and let $\varphi(W,x) = \chi(\sigma(W(x)))$. Suppose that:
\begin{itemize}
\item There exists an open subspace $O \subseteq \mathbb{R}^k$ containing $\sigma(0)$ where $\chi$ is affine with distinct non-vanishing coefficients i.e., $\chi(z) = \sum_i a_i z_i + b$ for $z \in O$ with $0 \not = a_i \not = a_j$ for $i \not = j$.
\item $\sigma \in C^2(\mathbb{C})$ and $\partial_z \partial_{\overline{z}} \sigma  (0) \not = 0$.  
\end{itemize}
Then $\varphi$ has unitary symmetries. 
\end{prop}  
We refer to the Appendix for a proof. Since typical (real-valued) deep neural networks have piece-wise linear activations functions such as (leaky) ReLU, they define piece-wise affine maps and therefore are affine when restricted to appropriate open subspaces. Moreover, the hypothesis on the coefficients $a_i$ in Proposition \ref{prop:deepnets} is \emph{generic}, meaning that it defines an open dense subset of $(a_1, \cdots, a_k) \in \mathbb{R}^k$. 

% {\color{gray}
% \subsubsection{Convolutional Networks}
% {\color{red}I would remove this section: it is shallow and the result has weird hypotheses.}

% Next, we discuss another popular model in machine learning: \emph{Convolutional Networks}. These have the form $\psi(W \star x)$, where $\star$ denotes the convolution (Equation \ref{eq:convol}) and $\psi \colon \free{G} \rightarrow Y$ is a map representing the head of the model that transforms the convolved input into the output. 

% \begin{prop}
% \label{lemm:convnet}
% Consider a map $\psi \colon \free{G} \rightarrow \mathcal{Y}$ and let $\varphi(W, x) = \psi(W \star x)
% $. Suppose that there exists $g \in G$ such that for all $x,y \in \free{G} $, if $\psi(x) = \psi(y)$ and $x_g =0$ then $y_g = 0$. Then $\varphi$ is unitarily injective. 
% \end{prop}
% \begin{proof}
%  Pick $W,W' \in \free{G}$ of the same norm such that $\varphi(W,x) = \varphi(W',x)$ for all $x \in \free{G}$. From the hypothesis on $\psi$ it follows that $(W \star x)_g$ vanishes if, and only if, $(W' \star x)_g$ does. By the arbitrariness of $x$, it follows that $W x $ vanishes if, and only if, $W' x $ does, and therefore $W$ and $W'$ share the same orthogonal complement. This implies that $W' = u W$ for some $u \in \mathbb{C} $ and since $W$ and $W'$ have the same norm, we conclude that $u \in \textnormal{U}(1)$.  
% \end{proof}
% }

% \subsection{Group Recovery}
% Proposition \ref{mainpropnc} enables to recover the group structure of $G$ (up to isomorphism) from the weight matrices $W_i$ of the unitarily injective maps involved. This addresses the problem of symmetry discovery discussed in Section \ref{sec:specrelwork} since it enables to recover an unknown group from (the weights of) an invariant model. To this end, assume that $\varphi_i$ satisfy the requirements of Proposition \ref{mainpropnc}. Moreover, we introduce the additional assumption that that $W_i(1) = 1 \in \textnormal{End}(V_i)$ for all $i$. If that's the case, $W$ coincides exactly with the Fourier transform by Proposition \ref{mainpropnc}. This implies that the multiplication table of $G$ can be recovered by: 
% % \end{proof}
% \begin{equation}\label{recoveryalg}
% gh = \underset{l\in G}{\textnormal{argmin}} \ \| W_{\bullet} (g) \odot  W_{\bullet}(h)  -   W_{\bullet} (l)   \|  \in \left\{ 0, \sqrt{2\underline{d}} \right\} ,
% \end{equation}
% where $\underline{d} = \sum_i d_i$ and  $\odot$ denotes the operator Hadamard product i.e., point-wise matrix multiplication.  \\

% Now, the multiplication table of $G$ is a discrete object, while the parameters $W$ of the model can vary continuously. Therefore, the invariance condition ($g \cdot W = W$ for all $g \in G$) can be related, while still recovering the multiplication table correctly. 



% \begin{prop}\label{mainrelax}
% Let $W \in \mathbb{C}^{d \times d}$, where $d = |G|$. Consider an activation function $\sigma : \ \mathbb{C} \to \mathbb{C}$ satisfying the following coercivity condition: there exist constants $C \in \mathbb{R}_{>0}$, $n \in \mathbb{N}$ such that for every $x \in \mathbb{C}$:
% \begin{equation}
% |\sigma(0) - \sigma(x)| \geq C \ |x|^n. 
% \end{equation}
% Suppose that for all $i$, $g\in G$, and $x \in \free{G}$ normal, the following holds: 
% \begin{equation}
% | \ \sigma ( W_i \ (g \cdot x) )  - \sigma(W_i \ x )  \ | < C \  \left(\frac{31}{256}\right)^{\frac{n}{2}}. 
% % | \ \omega_{\underline{i}}
% % (g \cdot x)  - \omega_{\underline{i}}
% % (x) \ | < \frac{31}{256  \sqrt{d}}. 
% \end{equation}
% % where $\omega_S{\underline{i}}$ is the map defined by Equation \ref{defomega}. 
% Suppose moreover that:
% \begin{itemize}
% \item $W$ is unitary w.r.t. the normalized scalar product i.e., $W W^{\dagger} = d \ 1$.
% \item $|W_{i,g}| = 1$ and $ W_{i,1} = 1$ for all $g,i$.   
% \end{itemize}
% Then Equation \ref{recoveryalg} holds.
% \end{prop}

% We refer to the Appendix for a proof. 




==> sections/3-theoretical-results_new.tex <==
\section{Theoretical Results}
\label{sec:theoretical-results}
We now present the primary theoretical contributions of this work. Concretely, we demonstrate that if certain parametric functions are invariant to a group then their weights must almost coincide with harmonics,  i.e. irreducible unitary group representations. We start by introducing general algebraic notions and principles, and then proceed to specialize them to machine learning scenarios. 

Let $G$ be a finite group, $\mathcal{H}$ be a set, and $V_1, \cdots, V_k$ be complex finite-dimensional Hilbert spaces. In what follows, we will consider the space
\begin{equation}
\mathcal{W} = \free{G} \otimes \bigoplus_i \textnormal{End}(V_i) \simeq \bigoplus_i \textnormal{End}(V_i)^{\oplus G}.
\end{equation}
$\mathcal{W}$ is a Hilbert space when endowed with the scalar product given by the product of the canonical scalar product over $\free{G}$ and the normalized Hilbert-Schmidt scalar products over $\textnormal{End}(V_i)$ (see Equation \ref{eq:hilbsch}). For $W \in \mathcal{W}$, we will denote each of its components as $W_i = (W_i(g))_g \in \textnormal{End}(V_i)^{\oplus G}$. Moreover, we will often interpret elements $W \in \mathcal{W}$ as linear maps $\free{G} \rightarrow \bigoplus_i \textnormal{End}(V_i)$ via $W(x) = \sum_{g \in G} W(g)x_g$ for $x \in \free{G}$, where $W(g) = (W_i(g))_i$. Note that $G$ acts on the left tensor factor of $\mathcal{W}$ while for each $i$, $\textnormal{U}(V_i)$ acts on the right tensor factor of $\free{G} \otimes \textnormal{End}(V_i)$ by composition of operators.     
\begin{defn}\label{def:symm}
We say that a map $\varphi \colon  \mathcal{W} \rightarrow \mathcal{H} $ has \emph{unitary symmetries} if for $W,W' \in \mathcal{W}$ of the same norm, $\varphi(W) = \varphi(W')$ implies that for each $i$ there exists a unitary operator $U_i \in \textnormal{U}(V_i)$ such that $W_i = U_i \cdot W_i'$.    
\end{defn}


In the context of machine learning, $\mathcal{H}$ will represent the \emph{hypothesis space}, consisting of functions the model can learn. On the other hand, $\varphi$ will represent the parametrization of such hypotheses, with its domain $\mathcal{W}$ being the space of weights. The component $\free{G}$ of $\mathcal{W}$ will be responsible for parametrizing the input space, while each component $\textnormal{End}(V_i)$ will represent a computational unit, i.e. a complex-valued \emph{neuron} in the language of neural networks. For commutative groups, we simply have $V_i = \mathbb{C} \simeq \textnormal{End}(V_i)$. In general, $\textnormal{End}(V_i)$ can be thought of as parametrizing matrix-valued signals, which, as mentioned in Section \ref{sec:overview}, are computed by neural units sometimes referred to as \emph{capsules} \cite{sabour2017dynamic}.  

The following is an abstract algebraic principle at the core of this work. 
\begin{thm}\label{prop:mainnew}
Suppose that $\varphi \colon \mathcal{W} \rightarrow \mathcal{H}$ has unitary symmetries and that for some $W \in \mathcal{W}$ the following holds:
\begin{itemize}
\item $\varphi(g \cdot W ) = \varphi(W)$ for all $g \in G$. 
\item $W_i$, seen as a linear map $\free{G} \rightarrow \textnormal{End}(V_i)$, is surjective for all $i$.
\end{itemize}
Then for every $i$ there exist $W_i' \in \textnormal{End}(V_i)$ and an irreducible unitary representation $\rho_i: \ G \rightarrow \textnormal{U}(V_i)$ such that for all $g \in G$,
\begin{equation}
W_i(g) = W_i' \rho_i(g)^\dagger. 
\end{equation}
\end{thm}
\begin{proof}
Since $\varphi$ has unitary symmetries and $\| g \cdot W \| = \| W \|$, it follows that for every $g \in G$ and every $i$ there exists $\rho_i(g) \in \textnormal{U}(V_i)$ such that
\begin{equation}\label{eq:generalw}
g \cdot W_i =  \rho_i(g) \cdot W_i . 
\end{equation}
In particular, by considering the component with index $1 \in G$ on both sides of Equation \ref{eq:generalw}, we see that $W_i(g^{-1}) = W_i(1) \ \rho_i(g)$. We wish to show that $\rho_i$ is a homomorphism. To this end, for all $g,h \in G$ it holds that
\begin{equation}\label{eq:generalproof}
 \rho_i(gh) \cdot W_i = (gh) \cdot W_i = g \cdot ( \rho_i(h) \cdot W_i ) = \rho_i(h) \cdot (g \cdot W_i)  = (\rho(g) \rho(h)) \cdot W_i.  
\end{equation}
By the surjectivity hypothesis, the set $\{W_i(g) \}_{g \in G}$ generates $\textnormal{End}(V_i)$ as a vector space. Therefore, Equation \ref{eq:generalproof} implies that $\rho_i(gh) = \rho_i(g) \rho_i(h)$, as desired. Lastly, note that $\rho_i$ is irreducible by the sujectivity assumption. Indeed, a nontrivial linear subspace of $V_i$ fixed by $\rho_i(g)$ for all $g$ would be sent by $W_i(g)$ into a fixed proper subspace due to Equation \ref{eq:generalw}. This contradicts the surjectivity of $W_i$. 
\end{proof}

Note that the surjectivity assumption implies the constraint $\sum_i \textnormal{dim}(V_i)^2 \leq |G|$. As a consequence of the result above, the full Fourier transform arises with an additional orthogonality assumption. 
\begin{cor}\label{mainpropnc}
Suppose that $\varphi \colon \mathcal{W} \rightarrow \mathcal{H}$ has unitary symmetries and that for some $W \in \mathcal{W}$ the following holds:
\begin{itemize}
\item $\varphi(g \cdot W ) = \varphi(W)$ for all $g \in G$. 
\item $W$ is unitary up to a multiplicative constant, i.e. $W^\dagger W = |G| I $. 
\end{itemize}
Then $W$ is the Fourier transform up to composing each of the components $W_i$ by an operator with Frobenius norm equal to $1$.
\end{cor} 
\begin{proof}
Note that the unitarity assumption above implies the surjectivity assumption from Theorem \ref{prop:mainnew}. Therefore, it follows that for every $i$, there exists an irreducible unitary representation $\rho_i : \ G \rightarrow \textnormal{U}(V_i)$ such that $W_i(g) = W_i(1) \ \rho_i(g)^\dagger$. We wish to show that if $i \not = j$ then $\rho_i$ and $\rho_j$ are non-isomorphic representations. If not, the orthogonality assumption implies that
\begin{align}   
0  = \sum_{g \in G}  \overline{W_i(g)} \otimes W_j(g)  & = \sum_{g \in G}  \left( \overline{W_i(1)} \otimes W_j(1)  \right) \left(  \rho_i(g)^{\top} \otimes \rho_j(g)^\dagger    \right) = \\
& =  |G| \  \overline{W_i(1)} \otimes W_j(1),
\end{align}
where $\top$ denotes the transpose and where the last identity follows from the Schur orthogonality relations. But then $W_i(1)$ or $ W_j(1)$ is vanishing, which contraddicts the unitarity assumption. 

Lastly, in order to compute the Frobenius norm of $W_i(1)$, note that 
\begin{equation}
|G| \ \| W_i(1) \|^2 = \sum_{g \in G} \| W_i(g) \ \rho_i(g) \|^2 = \sum_{g \in G} \| W_i(g) \|^2 = |G|,
\end{equation}
from which $\| W_i(1) \| = 1$ follows. 
\end{proof}
Again, the orthogonality assumption implies that $V_1, \cdots, V_k$ are the ambient Hilbert spaces of all the irreducible unitary representations of $G$ up to isomorphism, and in particular $\sum_i \textnormal{dim}(V_i)^2 = |G|$. 


We now wish to discuss the other crucial assumption of Theorem \ref{prop:mainnew} requiring that $\varphi(g \cdot W) = \varphi(W)$ for all $g \in G$, which is reminiscent of invariance. However, when $\mathcal{H}$ is a space of functions, we are typically interested in models that are invariant in the input variable rather than the weight variable. Therefore, we introduce the following condition, aimed at reconciling inputs and weights. To this end, suppose that $\mathcal{H}$ is a set of functions $\mathcal{X} \rightarrow \mathcal{Y}$, where $\mathcal{X}$ is a set acted upon by $G$ and $\mathcal{Y}$ is a set. We adhere to the notation $ \varphi(W, x) = \varphi(W)(x)$, $x \in \free{G}$, $W \in \mathcal{W}$, for simplicity.

\begin{defn}\label{defj:adj}
 We say that $\varphi$ satisfies the \emph{adjunction property} if
\begin{equation}
\varphi(W, g \cdot x) = \varphi(g^{-1} \cdot W, x) 
\end{equation}
for all $x\in \mathcal{X}, g \in G$. 
\end{defn}
The adjunction property implies that if $\varphi(W, x)$ is invariant in $x$, then $\varphi(g \cdot W, x) = \varphi(W, x)$ for all $x, g$, recovering the assumption of Theorem \ref{prop:mainnew}.

\begin{rmk}
As explained above, the tensor component $\free{G}$ of $\mathcal{W}$ typically represents the input space of a given machine learning model. One can consider the more general scenario when data consist of complex signals over a finite set $\mathcal{S}$ acted upon by $G$, therefore replacing $\free{G} = \mathbb{C}^G$ by $\mathbb{C}^\mathcal{S}$. This is the case, for example, for data consisting of images acted by the cyclic group via rotations, since the input space cannot be identified with signals over $G$. Assuming the action over $\mathcal{S}$ is \emph{free}, meaning that $g \cdot s = s$ implies $g=1$, $\mathcal{S}$ can be decomposed into copies of $G$ deemed \emph{orbits}. Specifically, there is an equivariant isomorphism $\mathcal{S} \simeq G \sqcup \cdots \sqcup G$, which in turn induces a linear isomorphism $\mathbb{C}^\mathcal{S} \simeq \free{G}^{\oplus p}$, where $p$ is the number of orbits. The results from this section can be extended to this scenario by applying all the arguments to the copies of $\free{G}$ separately, each of which will serve as a domain for its set of irreducible unitary representations. When the action is not free, it is necessary to take into account \emph{stabilizers}, i.e. $g \in G$ such that $g \cdot s = s$ for some $s \in \mathcal{S}$. Roughly speaking, we expect that the results from this section can be adapted to an extent, obtaining unitary representations `up to stabilizers'. However, the precise meaning of the latter has yet to be clarified, and goes beyond the scope of this work. 
\end{rmk}

\subsection{Examples}\label{sec:exmp}
In this section, we provide examples of machine learning models with unitary symmetries. As anticipated, in the context of machine learning $\mathcal{H}$ and $\mathcal{W}$ represent the hypothesis space and the parameter space, respectively. Indeed, in what follows $\mathcal{H}$ will consist of functions of the form $\free{G} \rightarrow \mathcal{Y}$ for some codomain $\mathcal{Y}$, and we will adhere to the notation from Definition \ref{defj:adj} accordingly. All the models considered in this section satisfy the adjunction property.

\subsubsection{Spectral Networks}\label{sec:specnet}
We start by considering \emph{Spectral Networks} -- a class of polynomial machine learning models that inspired this work\textemdash and to which our theory applies naturally. These models were introduced by \cite{sanborn2023bispectral} in cubic form based on the invariant theory of $\free{G}$ (see Section \ref{sec:specinv} in the Appendix for an overview of the latter). The overall idea behind Spectral Networks is to approximate the $n$-order polynomial invariants (deemed spectral invariants) of $\free{G}$ for an \emph{unknown} group $G$. Specifically, suppose that $V_1, \cdots, V_k$ are the ambient Hilbert spaces of the irreducible unitary representations of $G$. Given a multi-index $\underline{i} = (i_1, \cdots, i_n) \in \{1,  \cdots, k \}^n$, The Spectral Network of order $n$ is defined as the collection of parametric maps $\varphi_{\underline{i}}(W, \cdot):  \ \free{G}  \rightarrow \textnormal{End}(V_{i_1} \otimes \cdots \otimes V_{i_n})$: 
\begin{equation}\label{eq:ncspecnet}
\varphi_{\underline{i}}(W, x) =  W_{i_1} (x) \otimes \cdots \otimes W_{i_n}(x) \  \left( W_{i_1}^{\dagger} \odot   \cdots \odot W_{i_n}^{\dagger} \right) (\overline{x}),
\end{equation}
where $W=\oplus_iW_i \in \mathcal{W} = \free{G} \otimes  \oplus_i \textnormal{End}(V_i)$, $\odot$ denotes the $G$-wise tensor product of operators, and $\overline{x}$ denotes the component-wise conjugate of $x$. For a commutative $G$, since $V_i = \mathbb{C}$ for all $i$, the above expression reduces to:
\begin{equation}\label{bispecnet}
\varphi_{\underline{i}}(W, x) = W_{i_1}x  \cdots \ W_{i_n} x  \ \overline{W_{i_1} \odot \cdots \odot W_{i_n} \ x}.
\end{equation} 
 For $n=1$ Spectral Networks are deemed Power-Spectral Networks, and for a commutative $G$ they take the form $\varphi_i(W, x) = | W_i x |^2$. The latter can be simply interpreted as a linear model followed by an activation function. Even though the squared absolute value is uncommon as an activation function in machine learning, it has appeared in models of biological neural networks \cite{adelson1985spatiotemporal}. 

% On the same note, Spectral Networks for non-commutative groups can be defined as follows. Given a matrix $W \in \mathbb{C}^{d \times d}$, $d = |G|$, we think of it as a concatenation of $k$ tensors $W_i \in \mathbb{C}^{ d_i \times d_i \times d}$, where $d_1, \cdots, d_k$ are the dimensions of all the irreducible unitary representations of $G$. Given a multi-index $\underline{i} = (i_1, \cdots, i_n)$, we denote $d_{\underline{i}} = d_{i_1} \cdots d_{i_n}$. The \emph{Spectral Network} is then defined as the collection of parametric maps $\varphi_{\underline{i}}(W, \cdot):  \ \free{G} \simeq \mathbb{C}^d \rightarrow \mathbb{C}^{d_{\underline{i}} \times d_{\underline{i}}}$ given by: 
% \begin{equation}\label{eq:ncspecnet}
% \varphi_{\underline{i}}(W, x) =  ( W_{i_1} x )  \otimes \cdots \otimes (W_{i_n} x) \  \left( W_{i_1}^{\dagger} \overline{x} \ \otimes   \cdots \otimes W_{i_n}^{\dagger} \overline{x} \right).
% \end{equation}


For simplicity, we will consider only the Spectral Networks involving a single unitary representation; that is, we will focus on constant multi-indices $\underline{i} = (i, \cdots, i)$ in Equation \ref{eq:ncspecnet}. To this end, let $V$ be a finite-dimensional Hilbert space and $\mathcal{H}$ be the set of functions $\free{G} \rightarrow \textnormal{End}(V^{\otimes n})$ for some $n \in \mathbb{N}$. We set $\mathcal{W} = \free{G} \otimes \textnormal{End}(V)$. 
\begin{prop}\label{prop:specunitmain}
Consider the Spectral Network, given by:
\begin{equation}
\varphi(W, x) = W(x)^{\otimes n} \ W^{\dagger \odot n}(\overline{x}).
\end{equation}
Then $\varphi$ has unitary symmetries. 
\end{prop}
We refer to the Appendix for a proof. 


% We first focus on the commutative case, implying that $V = \mathbb{C}$ and therefore $W \in \free{G}$. Two examples of unitarily injective maps are: 
% \begin{itemize}
% \item \textit{Spectral Networks}: the model discussed in Section \ref{sec:specnet} obtained for a constant multi-index i.e.,
% \begin{equation}
% \varphi(W, x) = (Wx)^n \ \overline{W^{\odot n}x}
% \end{equation}
% for some $n > 0$. 
% \item \textit{McCulloch-Pitts Neurons}: a model of the form 
% \begin{equation}
%  \varphi(W,x) = \sigma(W x ),
% \end{equation}
% where $\sigma: \ \mathbb{C} \rightarrow \mathbb{C}$ is a map playing the role of an activation function. For $\sigma(z) = |z|^2$, this model reduces to a Spectral Network with $n=1$.    
% \end{itemize}

% Both the class of models above can be seen to satisfy the condition of unitarily injectivity, albeit with an assumption on $\sigma$.

\subsubsection{McCulloch-Pitts Neurons, Deep Networks, and Attention Mechanisms}

While Spectral Networks provide the most direct application of our theory, in this section we discuss the most common and fundamental neural network primitives in deep learning: the fully-connected McCulloch-Pitts neuron \cite{mcculloch1943logical}, the deep neural network, and the attention mechanism \cite{vaswani2017attention}. We consider models with complex coefficients and focus on commutative groups, i.e. all the Hilbert spaces $V_i$ from Definition \ref{def:symm} will be equal to $\mathbb{C}$. 

A McCulloch-Pitts neuron has the form $\varphi(W,x) = \sigma(W x )$, where $\sigma \colon \mathbb{C} \rightarrow \mathcal{Y}$ is a map playing the role of an activation function and $W \in \mathcal{W} = \free{G}$ is the weight vector. For $\sigma(z) = |z|^2$, the McCulloch-Pitts neuron reduces to a commutative Power-Spectral Network i.e., a Spectral Network with $n=1$.  The hypothesis space $\mathcal{H}$ consists of functions $\free{G} \rightarrow \mathcal{Y}$. 

\begin{prop}\label{lemm:mcculloch}
Consider a map $\sigma \colon \mathbb{C} \rightarrow \mathcal{Y}$ and let $\varphi(W,x) = \sigma(W x )$. Suppose that $0 \in \mathbb{C}$ is isolated in its fiber of $\sigma$, i.e. there exists an open subspace $O \subseteq \mathbb{C}$ such that $\sigma^{-1}(\sigma(0)) \cap O = \{ 0 \}$. Then $\varphi$ has unitary symmetries.
\end{prop}
We refer to the Appendix for a proof. The above assumption on $\sigma$ is satisfied by popular activations functions from neuroscience and machine learning, such as the sigmoid and the leaky Rectified Linear Unit (ReLU), applied after taking complex absolute value. 

% Next, we discuss the case of classical deep networks. We model the latter as $\varphi(W, x) = \chi(|W(x)|^2)$, where $W \in \mathcal{W} = \free{G} \otimes \mathbb{C}^k$ and $|\cdot|$ denotes the component-wise absolute value. Here, $k$ is the number of neurons in the first hidden layer of the network, while $\chi \colon \mathbb{R}_{\geq 0}^k \rightarrow \mathbb{R}$ is the head of the network, encompassing all the layers after the first one. Note that since typical neural networks are real-valued, we combine real and complex models. Namely, the first layer of $\varphi$ is complex, and its output is fed into the real head $\chi$ by taking squared absolute values. 

% % In what follows, we say that $\varphi(W,x)$ \emph{generically} has unitary hidden symmetries if Definition \ref{def:symm} holds for almost all $W \in \mathcal{W}$ i.e., if it holds in an open dense subspace of $\mathcal{W}$ (with the usual Euclidean topology). 
% Differently from Section \ref{sec:theoretical-results}, for the next result we will restrict $\mathcal{W}$ to the subspace of $\free{G} \otimes \mathbb{C}^k$ consisting of $W$ such that the components $W_i$ are orthonormal. This implies, in particular, the constraint $k \leq |G|$. Note that $\mathcal{W}$ is closed by the actions of $G$ and $\textnormal{U}(\mathbb{C})$. The orthonormality condition is anyway necessary in order to recover the full Fourier transform, as stated in Corollary \ref{mainpropnc}.  

% \begin{prop}\label{prop:deepnets}
% Suppose that there is an open subspace $O \subseteq \mathbb{R}_{\geq 0}^k$ containing $0$ where $\chi$ is affine with distinct non-vanishing coefficients i.e., $\chi(z) = \sum_i a_i z_i + b$ for $z \in O$ with $0 \not = a_i \not = a_j$ for $i \not = j$. Then $\varphi(W, x) = \chi(|W(x)|^2)$ has unitary symmetries. 
% \end{prop}  
% We refer to the Appendix for a proof. Since typical (real-valued) deep neural networks have piece-wise linear activations functions such as (leaky) ReLU, they define piece-wise affine maps and therefore are affine when restricted to appropriate open subspaces. Moreover, the hypothesis on the coefficients $a_i$ in Proposition \ref{prop:deepnets} is \emph{generic}, meaning that it defines an open dense subset of $(a_1, \cdots, a_k) \in \mathbb{R}^k$. 


Next, we discuss the case of classical deep networks. We model the latter as $\varphi(W, x) = \chi(\sigma(W(x)))$, where $W \in \mathcal{W} = \free{G} \otimes \mathbb{C}^k$ and $\sigma\colon \mathbb{C} \rightarrow \mathbb{R}$ represents the activation function, computed coordinate-wise on $\mathbb{C}^k$. Here, $k$ is the number of neurons in the first hidden layer of the network, while $\chi \colon \mathbb{R}^k \rightarrow \mathbb{R}$ is the head of the network, encompassing all the layers after the first one. Note that since typical neural networks are real-valued, we combine real and complex models. Namely, the first layer of $\varphi$ is complex, and its output is fed into the real head $\chi$ by applying the activation function. 

Differently from Section \ref{sec:theoretical-results}, for the next result we will restrict $\mathcal{W}$ to the subspace of $\free{G} \otimes \mathbb{C}^k$ consisting of $W$ such that the components $W_i$ are orthonormal. This implies, in particular, the constraint $k \leq |G|$. Note that $\mathcal{W}$ is closed by the actions of $G$ and $\textnormal{U}(\mathbb{C})$. The orthonormality condition is anyway necessary in order to recover the full Fourier transform, as stated in Corollary \ref{mainpropnc}.  

\begin{prop}\label{prop:deepnets}
Consider maps $\sigma \colon \mathbb{C} \rightarrow \mathbb{R}$, $\chi \colon \mathbb{R}^k \rightarrow \mathbb{R}$ and let $\varphi(W,x) = \chi(\sigma(W(x)))$. Suppose that:
\begin{itemize}
\item There exists an open subspace $O \subseteq \mathbb{R}^k$ containing $\sigma(0)$ where $\chi$ is affine with distinct non-vanishing coefficients i.e., $\chi(z) = \sum_i a_i z_i + b$ for $z \in O$ with $0 \not = a_i \not = a_j$ for $i \not = j$.
\item $\sigma \in C^2(\mathbb{C})$ and $\partial_z \partial_{\overline{z}} \sigma  (0) \not = 0$.  
\end{itemize}
Then $\varphi$ has unitary symmetries. 
\end{prop}  
We refer to the Appendix for a proof. Since typical (real-valued) deep neural networks have piece-wise linear activations functions such as (leaky) ReLU, they define piece-wise affine maps and therefore are affine when restricted to appropriate open subspaces. Moreover, the hypothesis on the coefficients $a_i$ in Proposition \ref{prop:deepnets} is \emph{generic}, meaning that it defines an open dense subset of $(a_1, \cdots, a_k) \in \mathbb{R}^k$. 

Lastly, we focus on a popular model that is ubiquitous in sequence processing and computer vision: the self-attention mechanism. We consider complex-valued attention blocks \cite{kothapally2022complex} and, for simplicity, assume that the queries, keys and values are one-dimensional. The inputs of the model consist of sequences of signals over $G$, i.e. the input space is $\free{G} \otimes \mathbb{C}^T$, where $T$ is the sequence length. The weight space is $\mathcal{W} = \free{G} \otimes \mathbb{C}^3 \simeq  \free{G} \oplus \free{G} \oplus \free{G}$. Here, the three summands represent weights for queries, keys, and values respectively. The attention block $\varphi(W, \cdot) \colon \free{G} \otimes  \mathbb{C}^T \rightarrow \mathcal{Y} = \mathbb{C}^T$ is defined for $x = (x_i)_{1 \leq i \leq T}$ and $W  = (Q, K, V)$ as: 
\begin{equation}\label{eq:attn}
\varphi(W,x)_i = \sum_j \frac{e^{|Qx_i Kx_j|}}{\sum_k e^{|Qx_i Kx_k|}} \ V x_j, \hspace{3em} i=1, \cdots, T.
\end{equation}
Note that, by convention, we set to $1$ all the traditional hyperparameters such as temperature and scaling. 

\begin{prop}\label{prop:attn}
If $T > 1$, the map defined by $\varphi$ in Equation \ref{eq:attn} has unitary symmetries.   
\end{prop}

We refer to the Appendix for a proof. 

\begin{rmk}
Proposition \ref{prop:attn} extends to \emph{graph} attention mechanisms \cite{velickovic2017graph}, where the indices of the sums in Equation \ref{eq:attn} run over neighbors of $i$, according to a given undirected graph structure on $T$ nodes. Assuming the graph is non-trivial (i.e, contains at least one edge), our proof extends verbatim to this more general setting. 
\end{rmk}

% Next, we discuss another popular model in machine learning: \emph{Convolutional Networks}. These have the form $\psi(W \star x)$, where $\star$ denotes the convolution (Equation \ref{eq:convol}) and $\psi \colon \free{G} \rightarrow Y$ is a map representing the head of the model that transforms the convolved input into the output. 

% \begin{prop}
% \label{lemm:convnet}
% Consider a map $\psi \colon \free{G} \rightarrow \mathcal{Y}$ and let $\varphi(W, x) = \psi(W \star x)
% $. Suppose that there exists $g \in G$ such that for all $x,y \in \free{G} $, if $\psi(x) = \psi(y)$ and $x_g =0$ then $y_g = 0$. Then $\varphi$ is unitarily injective. 
% \end{prop}
% \begin{proof}
%  Pick $W,W' \in \free{G}$ of the same norm such that $\varphi(W,x) = \varphi(W',x)$ for all $x \in \free{G}$. From the hypothesis on $\psi$ it follows that $(W \star x)_g$ vanishes if, and only if, $(W' \star x)_g$ does. By the arbitrariness of $x$, it follows that $W x $ vanishes if, and only if, $W' x $ does, and therefore $W$ and $W'$ share the same orthogonal complement. This implies that $W' = u W$ for some $u \in \mathbb{C} $ and since $W$ and $W'$ have the same norm, we conclude that $u \in \textnormal{U}(1)$.  
% \end{proof}
% }

% \subsection{Group Recovery}
% Proposition \ref{mainpropnc} enables to recover the group structure of $G$ (up to isomorphism) from the weight matrices $W_i$ of the unitarily injective maps involved. This addresses the problem of symmetry discovery discussed in Section \ref{sec:specrelwork} since it enables to recover an unknown group from (the weights of) an invariant model. To this end, assume that $\varphi_i$ satisfy the requirements of Proposition \ref{mainpropnc}. Moreover, we introduce the additional assumption that that $W_i(1) = 1 \in \textnormal{End}(V_i)$ for all $i$. If that's the case, $W$ coincides exactly with the Fourier transform by Proposition \ref{mainpropnc}. This implies that the multiplication table of $G$ can be recovered by: 
% % \end{proof}
% \begin{equation}\label{recoveryalg}
% gh = \underset{l\in G}{\textnormal{argmin}} \ \| W_{\bullet} (g) \odot  W_{\bullet}(h)  -   W_{\bullet} (l)   \|  \in \left\{ 0, \sqrt{2\underline{d}} \right\} ,
% \end{equation}
% where $\underline{d} = \sum_i d_i$ and  $\odot$ denotes the operator Hadamard product i.e., point-wise matrix multiplication.  \\

% Now, the multiplication table of $G$ is a discrete object, while the parameters $W$ of the model can vary continuously. Therefore, the invariance condition ($g \cdot W = W$ for all $g \in G$) can be related, while still recovering the multiplication table correctly. 



% \begin{prop}\label{mainrelax}
% Let $W \in \mathbb{C}^{d \times d}$, where $d = |G|$. Consider an activation function $\sigma : \ \mathbb{C} \to \mathbb{C}$ satisfying the following coercivity condition: there exist constants $C \in \mathbb{R}_{>0}$, $n \in \mathbb{N}$ such that for every $x \in \mathbb{C}$:
% \begin{equation}
% |\sigma(0) - \sigma(x)| \geq C \ |x|^n. 
% \end{equation}
% Suppose that for all $i$, $g\in G$, and $x \in \free{G}$ normal, the following holds: 
% \begin{equation}
% | \ \sigma ( W_i \ (g \cdot x) )  - \sigma(W_i \ x )  \ | < C \  \left(\frac{31}{256}\right)^{\frac{n}{2}}. 
% % | \ \omega_{\underline{i}}
% % (g \cdot x)  - \omega_{\underline{i}}
% % (x) \ | < \frac{31}{256  \sqrt{d}}. 
% \end{equation}
% % where $\omega_S{\underline{i}}$ is the map defined by Equation \ref{defomega}. 
% Suppose moreover that:
% \begin{itemize}
% \item $W$ is unitary w.r.t. the normalized scalar product i.e., $W W^{\dagger} = d \ 1$.
% \item $|W_{i,g}| = 1$ and $ W_{i,1} = 1$ for all $g,i$.   
% \end{itemize}
% Then Equation \ref{recoveryalg} holds.
% \end{prop}

% We refer to the Appendix for a proof. 




==> sections/3b-group-recovery.tex <==

\subsection{Group Recovery}\label{sec:grrecov}
Corollary \ref{mainpropnc} allows us to recover the group structure of $G$ up to isomorphism from the weights of a map with unitary symmetries. In other words, this enables the recovery of an unknown group in a data-driven manner from the weights of an invariant machine learning model, addressing the problem of symmetry discovery discussed in Section \ref{sec:overview}. The procedure was originally suggested and validated empirically in \cite{sanborn2023bispectral}. 

To this end, assume that $\varphi_i$ satisfies the requirements of Corollary \ref{mainpropnc}. Moreover, we introduce the additional assumption that $W_i(1) = I \in \textnormal{End}(V_i)$ for all $i$. If that is the case, $W$ coincides exactly with the Fourier transform by Corollary \ref{mainpropnc}. This implies that the multiplication table of $G$ can be recovered by: 
%\end{proof}
\begin{equation}\label{recoveryalg}
gh = \underset{l\in G}{\textnormal{argmin}} \ \| W(g) \odot  W(h)  -   W (l)   \|,
\end{equation}
where  $\odot$ denotes the Hadamard product i.e., component-wise operator composition. Note that this notation has a different meaning here than in Section \ref{sec:specnet}. Since the $W(g)$'s are orthogonal, the only possible values for the norms over which the minimum is performed are $0$ and $\sqrt{2 |G|}$.

The multiplication table of $G$ is a discrete object, while the weights $W \in \mathcal{W}$ can vary continuously. Therefore, it is natural to expect that the invariance condition ($g \cdot W = W$ for all $g \in G$) can be relaxed, while still recovering the multiplication table correctly. In what follows, we analyze relaxations of invariance and give bounds in which the group recovery algorithm holds. We start by introducing a quantity measuring how close a map is to having unitary symmetries. To this end, we assume that $\mathcal{H}$ is a metric space with distance function $\Delta: \mathcal{H} \times \mathcal{H} \rightarrow \mathbb{R}_{\geq 0}$. 
\begin{defn}
Given a map $\varphi \colon \mathcal{W} \rightarrow \mathcal{H} $, its \emph{unitarity defect} is defined for $\delta \in \mathbb{R}_{>0}$ as: 
\begin{equation}
\omega_\varphi(\delta) = \sup_{\substack{W, W' \in \mathcal{W} \\ \| W \| = \| W' \| \\ \Delta(\varphi(W), \varphi(W')) \leq \delta}} \max_i \quad \inf_{U \in \textnormal{U}(V_i)} \quad \| W_i - U \cdot W_i'  \|  , 
\end{equation}
% where the supremum runs over all the $W, W' \in  \free{G} \otimes \textnormal{End}(V)$ of the same norm such that $\Delta(\varphi(W),  \varphi(W')) \leq \delta$ while the infimum runs over $U \in \textnormal{U}(V)$.
\end{defn}
Note that $\varphi$ has unitary symmetry if, and only if, $\omega_\varphi(0) = 0$. The following is our main relaxation result. 
\begin{thm}\label{prop:mainrelax}
Suppose that $\varphi \colon \mathcal{W} \rightarrow \mathcal{H}$ is a map and fix $W \in \mathcal{W}$. Denote 
\begin{equation}
L = \| W^\dagger W - |G|I \|_\infty,
\end{equation}
where $\| \cdot \|_\infty$ is the uniform Frobenius norm for $G \times G$ matrices. Suppose that the following holds:
\begin{itemize}
 \item  For all $g\in G$:
 \begin{equation}\label{eq:moduludbound}
 \omega_{\varphi} \left( \Delta(\varphi(g \cdot W), \varphi(W)) \right) < \frac{\sqrt{\frac{1}{2} - \frac{L}{|G|}}}{\sqrt{|G| + L} + 1} 
 \end{equation}
% \item $W$ is unitary up to a multiplicative constant i.e., $W^\dagger W = |G| \ 1 $. 
\item $L \leq \frac{|G|}{2} .$
\item $W_i(1) = I \in \textnormal{End}(V_i)$ for all $i$. 
\end{itemize}

Then Equation \ref{recoveryalg} holds, i.e. the group recovery algorithm is correct.    
\end{thm}
\begin{proof}
Firstly, the definition of $L$ implies the inequalities $|G| - L \leq \| W(g)\|^2 \leq |G| + L$ and $|\langle W(g), W(h)\rangle| \leq L$ for all $g,h \in G$. In particular, 
\begin{equation}
\|W(g) - W(h )\|^2 = \| W(g)\|^2 + \| W(h) \|^2 -2 \textnormal{Re}(\langle W(g), W(g) \rangle) \geq 2 |G| - 4L. 
\end{equation}
By hypothesis, for each $i$ and $g \in G$ there exists $\rho_i(g) \in \textrm{U}(V_i)$ such that 
\begin{equation}\label{ineqc}
\| g^{-1} \cdot W_i - \rho_i(g) \cdot W_i \| < \frac{\sqrt{\frac{1}{2} - \frac{L}{|G|}}}{\sqrt{|G| + L} + 1}. 
\end{equation}
In particular, $\|  W_{i}(gh) - \rho_i(g)W_{i}(h)   \|$ is bounded by the same quantity for all $g,h \in G$. Therefore, via the triangle inequality we see that:
\begin{align}\label{ineqfinal}
& \| W_{i}(g)W_{i}(h) - W_{i}(gh) \| \leq \\
\leq & \|W_{i}(h) W_{i}(g) - \rho_i(g) W_{i}(h)\| + \| W_{i}(gh) - \rho_i(g)W_{i}(h) \| = \\
= & \underbrace{\|W_{i}(h)\|}_{\leq \sqrt{|G| + L}} \ \|W_{i}(g) - \rho_i(g)W_{i}(1) \|  + \| W_{i}(gh) - \rho_i(g)W_{i}(h) \| < \\ 
< & \sqrt{\frac{1}{2} - \frac{L}{|G|}}.
\end{align}
Equation \ref{ineqfinal} implies that 
\begin{equation}
\| W(g) \odot W(h) - W(gh)  \| < \sqrt{|G|}\sqrt{\frac{1}{2} - \frac{L}{|G|}} = \frac{\sqrt{2|G| - 4L}}{2}.
\end{equation}
Since $\|  W(p)  - W(q)  \| \geq \sqrt{2|G| -4L}$ for all $p \not = q \in G$, $W(g) \odot W(h)$ is closer to $W(gh)$ than to any other $W(q)$ for $q \in G$, which immediately implies the desired result. 
\end{proof}
The assumption on $L$ in the above result is a relaxation of the unitarity assumption in Corollary \ref{mainpropnc} since $L=0$ if, and only if, $W$ is unitary up to a multiplicative constant. 

We provide an explicit bound for the unitarity defect of the McCulloch-Pitts neurons discussed in Section \ref{sec:exmp}. To this end, let $\mathcal{H}$ be the space of continuous functions defined on the unit sphere in $\free{G}$ equipped with the uniform metric (i.e., the $L_\infty$ distance) as $\Delta$. 
\begin{prop}\label{prop:modulusculloch}
Let $W \in \free{G}$ and consider $\varphi(W,x) = \sigma(W x)$. Suppose that the activation function $\sigma \colon \mathbb{C} \to \mathbb{C}$ is continuous and satisfies the following coercivity condition: there exist constants $C \in \mathbb{R}_{>0}$, $n \in \mathbb{N}$ such that for every $x \in \mathbb{C}$:
\begin{equation}
|\sigma(0) - \sigma(x)| \geq C \ |x|^n. 
\end{equation}
Then the unitarity defect of $\varphi$  satisfies for $\delta < C$: 
\begin{equation}\label{eq:mccullochbound}
\omega_\varphi(\delta)  \leq \sqrt{2\left( 1- \sqrt{1 -  \left( \frac{\delta}{C} \right)^{\frac{2}{n}}} \right) }. 
\end{equation}
\end{prop}
We refer to the Appendix for a proof. Note that the coercivity condition from above plays the role of the assumption on $\sigma$ from Proposition \ref{lemm:mcculloch}.

% By combining the two bounds from Equation \ref{eq:moduludbound} and Equation \ref{eq:mccullochbound} we get a bound on the distance in $\mathcal{H}$ within which the group recovery is correct: {\color{red}Continue}


% \subsection{A Note on Locality}
% All of our results so far revolve around harmonics over $G$. However, the weights observed in practice of both biological and artificial neural networks resemble localized harmonics i.e., \emph{Gabor wavelets}. The latter can be defined in general as a point-wise product $\rho \odot \pi$, where $\pi$ is a (non-normalized) density function over $G$ and $\rho: G \rightarrow \textnormal{U}(V)$ is an irreducible unitary representation. The traditional Gabor wavelets correspond to the case where $G = \mathbb{R}^n$ and $\pi$ is Gaussian density. In this section, we sketch an extension of our main result to localized harmonics. Specifically, we argue that the latter emerge from a local version of the invariance property.  \\

% For simplicity, we focus on a `hard' notion of locality, meaning that $\pi = \chi_A \in \{0,1 \}^G$ is the characteristic function of a subset $A \subseteq G$, and therefore $\pi \odot \rho$ confines the support of $\rho$ to $A$. Given $A$, we introduce the following localized relation: $W,W' \in \free{G} \otimes \textnormal{End}(V)$ are related (written $W \triangleleft W'$) if $\chi_A \odot (g \cdot W) = \chi_A \odot  W'$ for some $g \in G$. In other words, $W$ and $W'$ coincide on $A$ up to acting by $G$ on $W'$. Based on this, we state Proposition \ref{prop:mainnew} in its localized version. 

% \begin{prop}\label{prop:mainlocal}
% Let $\varphi: \ \free{G} \otimes \textnormal{End}(V) \rightarrow \mathcal{H}$ be a unitarily injective map. Suppose that for some $W \in \free{G} \otimes \textnormal{End}(V)$ the following holds:
% \begin{itemize}
% \item $\varphi(W ) = \varphi(W')$ for all $W'$ such that $W \triangleleft W'$.  
% \item $W$, seen as a linear map $\free{G} \rightarrow \textnormal{End}(V)$, is surjective.
% \end{itemize}
% Then there exist $W' \in \textnormal{End}(V)$ and an irreducible unitary representation $\rho: \ G \rightarrow \textnormal{U}(V)$ such that for all $g \in G$
% \begin{equation}
% W(g) = \chi_A(g) \ W' \rho(g)^\dagger. 
% \end{equation}
% \end{prop}

% \begin{proof}
% By unitarily injectivity, if $W'$ coincides with $W$ on $A$ then $W = U \cdot W'$ for some $U \in \textnormal{U}(V)$. This implies that  From here on, the proof follows the same lines as the one of Proposition \ref{prop:mainnew}. 
% \end{proof}






==> sections/4-experimental-results.tex <==
\subsubsection{Implementation}


\begin{figure}[t]
\centering
    \begin{subfigure}[b]{.30\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/c6-labeled.png}
        \subcaption*{$C_6 \simeq C_2 \times C_3$}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}[b]{.30\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/c2cube.png}
        \subcaption*{$C_2 \times C_2 \times C_2$}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}[b]{.30\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/dh3.png}
        \subcaption*{$D_3 \simeq S_3$}
    \end{subfigure}
\caption{\textbf{Learned Group Multiplication Tables.} Tables inferred by Power-Spectral Networks for the groups $C_6$ (commutative), $C_2 \times C_2 \times C_2$ (commutative), and $D_3$ (non-commutative).  Rows and columns are labeled with integers that index group elements. Each cell of the table contains the index of the group element obtained by composing the group elements indexed in the row and column.  Note that the table is a symmetric matrix if, and only if, the group is commutative.} 
\label{fig:cayley}
\end{figure}


\label{sec:experimental-results}
We now empirically explore the theory developed in this paper and demonstrate that Spectral Networks are able to recover the group structure in practice. To this end, we implement a non-commutative Power-Spectral Network $\varphi_i(W, x) = W_ix \ W^\dagger_i \overline{x}$ with weights $W \in \mathbb{C}^{d_i \times d_i \times d}$, where $d = |G|$ is the cardinality of the given group and $d_1, \cdots, d_k$ are the dimensions of its irreducible unitary representations. As discussed at the beginning of Section \ref{sec:grrecov}, we force $W_i(1) = I \in \mathbb{C}^{d_i \times d_i}$, where the index $1$ is arbitrarily chosen. 

Following \cite{sanborn2023bispectral}, we train the model via \emph{contrastive learning} \cite{jaiswal2020survey}. Namely, given a finite dataset $\mathcal{D}$ of pairs $(x,y)$, where $x,y \in \free{G} \simeq  \mathbb{C}^d$ and $x = g \cdot y$ for an unknown $g \in G$, the objective optimized by the model is:
\begin{equation}\label{eq:objcomm}
\mathcal{L}(W) = \sum_{(x,y) \in \mathcal{D}} \sum_{i} \ \|\varphi_{i}(W, x) - \varphi_{i}(W, y) \|^2 + \eta \ \|dI    -  W W^\dagger  \|^2 , 
\end{equation}
where $\eta > 0$ is a hyper-parameter and $\| \cdot \|$ is the Frobenius norm. The first term in Equation \ref{eq:objcomm} encourages invariance with respect to $G$ while the second one encourages $W$ to be unitary. 

The model is trained via the Adam optimizer \cite{kingma2014adam}, which interprets the complex weights as real tensors of doubled dimensionality. The dataset $\mathcal{D} \subseteq \free{G}\oplus \free{G} $ is generated procedurally by first sampling $x$ from a standard Gaussian distribution over $\free{G} \simeq \mathbb{R}^{2d}$, then sampling $g \in G$ uniformly, and finally producing the datapoint $(x,y=g \cdot x) \in \mathcal{D}$. We provide a Python implementation of both the model and the experiments at a public repository (see Section \ref{sec:overview}). The code is available in both the PyTorch \cite{NEURIPS2019_9015} and the JAX \cite{jax2018github} frameworks. 


\begin{figure}[h]
\centering
    \begin{subfigure}[b]{.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/c5-zoom-light-2.pdf}
        \subcaption*{$C_5$}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}[b]{.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/c6-zoom-light-2.pdf}
        \subcaption*{$C_6$}
    \end{subfigure}
\caption{\textbf{Group Recovery Accuracy.} Accuracy for the recovery of the group multiplication tables across $20$ training runs as the amount of noise injected into data increases. The transition from $1.0$ to $0.0$ accuracy is sharp, and here we visualize only the noise regions where the values are non-trivial. } 
\label{fig:cayleybars}
\end{figure}

Once trained, we evaluate the model by checking whether the multiplication table $M \in \{1, \cdots, d \}^{d\times d}$ obtained via the group recovery algorithm described by Equation \ref{recoveryalg} coincides with the one of $G$. Since there is no canonical ordering on $G$, the table is recovered up to a permutation $\pi$ of $\{1, \cdots, d \}$ acting as $(\pi \cdot M)_{i,j} = \pi(M_{\pi^{-1}(i), \pi^{-1}(j)})$. Therefore, we check whether $\pi \cdot M$ coincides with the table of $G$ for all the permutations $\pi$. Figure \ref{fig:cayley} reports the (correct) multiplication tables obtained at convergence for both commutative and non-commutative groups. Specifically, we consider the cyclic group $C_6$, the product of cyclic groups $C_2 \times C_2 \times C_2$ and the dihedral group $D_3$, which is isomorphic to the symmetric group $S_3$. 

In order to validate empirically the robustness of the group recovery procedure, we additionally train the model on data corrupted by white noise, i.e. $\mathcal{D}$ consists of pairs $(x, y = g \cdot x + \epsilon)$, where $\epsilon$ is sampled from an isotropic Gaussian distribution. We vary the standard deviation of the latter and report in Figure \ref{fig:cayleybars} the number of times the multiplication table is recovered correctly across $20$ training runs -- a metric referred to as `table accuracy'. 

As can be seen, the group structure is recovered most of the times even with large amounts of noise -- up to $\sim 0.5$ standard deviation. The performance quickly degrades as the noise reaches a critical threshold. This demonstrates empirically that the group recovery procedure is robust to noise, which is in line with the theoretical bounds from Theorem \ref{prop:mainrelax}.  



% TODO:

% \begin{enumerate}
%     \item Explain results in text
%     \item Run results over many random seeds \& quantify
%     \item Compare learned irreps to analytical irreps
%     \item Group recovery under noise
% \end{enumerate}


% \subsection{Power Spectral Networks}

% Informed by the proof of Proposition \ref{mainproppower}, we propose a novel neural network architecture, which we call \textit{Power Spectral Networks}, for learning the irreducible representations of commutative groups. Prior work \cite{sanborn2023bispectral} has proposed a neural network architecture based on the ansatz of the bispectrum\textemdash the unique third-order polynomial invariant\textemdash and demonstrated that the weights of the network converge to a $G$-Fourier matrix as the network learns to collapse signal orbits. Proposition \ref{mainproppower} implies that the same should be observed in a second-order network that mirrors the ansatz of the power spectrum\textemdash the unique second-order polynomial invariant. As a second-order model, the Power Spectral Network has the advantage of being simpler to implement, compute, and train. 

% \textbf{Power Spectral Networks} are defined by a single linear layer $z = Wx$ parameterized by weight matrix $W \in \mathbb{C}^{n \times n}$. The linear layer is followed by the second-order transform:

% \begin{equation}
%     \phi = z^{\dagger}z
% \end{equation}

% Power Spectral Networks are trained with the Orbit Separation loss from \cite{sanborn2023bispectral}: 

% \begin{equation}
%     L(x_a) = \sum_{j | y_b = y_a}\| \bar{\beta}(x_a) - \bar{\beta}(x_b) \|_2^2 + \gamma \| x_a - W^{\dagger}W\,x_a\|_2^2.
% \label{eq:loss-function}
% \end{equation}

% [add the mean innovation].

% [In addition, we add an explicit regularization penality]

% The uniqueness of the power spectrum as a second-order invariant guarantees that the weights in a Power Spectral Network will converge to a $G$-Fourier matrix if the network learns to output a $G$-invariant map. 


% \subsection{Learning Irreducible Representation with Power Spectral Networks}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/dist-temp.png}
%     \caption{(\textbf{Temporary}) [Figure showing closeness of learned features to Fourier filters on the y axis with amount of input noise on the x-axis]}
%     \label{fig:feature-examples}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{figs/weights-real-temp.png}
%     \includegraphics[width=\linewidth]{figs/weights-imag-temp.png}
%     \caption{(\textbf{Temporary}) [Figure showing learned Fourier matrices]}
%     \label{fig:learned-weights}
% \end{figure}

% \subsection{Recovering Cayley Tables}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.6\textwidth]{example-image-a}
%     \caption{[Figure showing Cayley table success rate]}
%     \label{fig:cayley-tables}
% \end{figure}



==> sections/5-discussion.tex <==
\section{Conclusions, Limitations, and Future Work}
\label{sec:discussion}

In this work, we proved that if a machine learning model of a certain kind is invariant to a finite group, then its weights are closely related to the Fourier transform on that group. We discussed how, as a consequence, the algebraic structure of an unknown group can be recovered from a model that is invariant. We established these results for both commutative and non-commutative groups, and discussed relaxed conditions under which the group recovery procedure holds. Our results represent a first step towards a mathematical explanation of universal features inferred by both biological and artificial neural networks. 

Due to its open-ended nature, this work is subject to a number of limitations and leaves directions open for future investigation. First,  our theory encompasses models with complex-valued weights, which are non-canonical in machine learning. Thus, exploring analogues of the theory over real numbers is an interesting direction that would fit more directly with current practices in the field. 

In addition, our theoretical framework encompasses learning models with unitary symmetries. The latter is a technical property satisfied by Spectral Networks and, to an extent, by traditional deep networks. However, it is not clear what other models fit into our framework, and whether the notion is general enough to accommodate other computational primitives fundamental to machine learning, such as the attention mechanisms. This is an open question that is worthy of investigation. 

Lastly, in this work we focused on groups and their associated harmonics. However, the representations within neural networks or biological systems often resemble imperfect, or \textit{localized}, versions of harmonics, i.e. wavelets, such as Gabors. Since wavelets do not describe group homomorphisms, our theory would need to be extended to accommodate this kind of locality. We suspect that this may be achieved by generalizing the framework to \emph{groupoids} -- an algebraic group-like structure that formalizes a locally-defined composition. This, however, goes beyond the scope of our work, and we leave it for future research. 

\section*{Acknowledgements}
This work was supported by the Swedish Research Council, the Knut and Alice Wallenberg Foundation and the European Research Council (ERC-BIRD-884807).
\newpage 

==> sections/intro_invariant_theory.tex <==
\section{What is invariant theory?}
% The remarkable transformation-invariance properties of the familiar power spectrum and bispectrum arise from a branch of mathematics known as \textit{invariant theory}. 

% Broadly, the project of invariant theory is to understand functions which are invariant to group transformations. Typically, the functions considered are polynomials of a given degree.

% What is the set of polynomials which are unchanged when the input variables are transformed by group actions?

% \textbf{Invariant theory} \\
% * I think it would be good for us to write an extremely approachable, high-level intro to what invariant theory is about, give some simple examples, then build up from there to the power spectral and bispectral invariants. \\
% I think we could do this by saying what it's about at a high-level: \\
% * What is the set of polynomials that are unchanged when applying a group transformation to the input variables? Here we could give a simple example with a discrete group acting on the plane. From there, we could build up (ideally with intuitive arguments alone) to the power spectrum, then to the bispectrum. Perhaps from there we can introduce, at a high level, the contribution of the proof in these simpler terms. I think from there, we have the technical section which is buttoned up tight proving the theorems for the commutative and noncommutative cases. Following that, I think we should have a nice transitional paragraph that reminds the reader the significance of the theorem (1) in terms of the intuition given above and (2) in terms of the implications for learning groups from data (i.e. to our original paper and for learning the irreps using the power spectrum). Reinforce the point about uniqueness.

% From here, I think we should switch to the algorithmic/numerical side of things, first introducing the power spectral network, what we expect to be learned and why, etc. This will be followed by the computational wins in terms of the better scaling to input images ($n$ vs $n^2$), empirical measures of compute cost (e.g. time), along with the speedup that comes from using the mean version of the loss instead of the pairwise distance.

\textit{Invariant theory motivation + intro.} 
The remarkable transformation-invariance properties of the familiar power spectrum and bispectrum arise from a branch of mathematics known as \textit{invariant theory}. 
% Invariant theory is a branch of mathematics that provides a powerful framework for understanding the transformation structure of groups and their connection to group-invariant maps. 
Broadly, the project of invariant theory is to understand how functions, typically polynomials, behave under group transformations of their variables. This theory allows us to recast the question of constructing group-invariant neural networks into a question about sets of polynomials which are left unchanged when their input variables are transformed.

% A fundamental question in invariant theory is how to construct polynomials that remain unchanged under these group transformations. 

\textit{Intuitive Examples.} 
To illustrate this idea, let's consider two simple examples. Consider points in the plane with coordinates $x = (x_1,x_2)$. We can construct group transformations that operate on these points, such as permutations $(x_1,x_2) \mapsto (x_2,x1)$ or rotations $x \mapsto Rx$, where $R$ is a rotation matrix. Note that the polynomial $f(x,y) = x^2 + y^2$ is invariant to both group transformations.

\textit{The Symmetric Polynomials.}
One notable class of invariant polynomials is the set of \textit{symmetric polynomials}, the set of polynomials invariant under arbitrary permutation of their input variables. (add a few examples and non-examples).

% By examining the properties of such polynomials, we can gain insights into the underlying group structure and its impact on the invariance of mathematical objects.

\textit{Setting up the framing for the power spectrum: quadratic forms / polynomials}
In the realm of machine learning, we are often interested in constructing invariant maps for signals or images undergoing transformations. Take, for example, a real-valued signal in time sampled at $n$ discrete points under cyclic translation, $x = (x_1, x_2, ..., x_n)$. 

How can we construct a polynomial invariant to cyclic translation? Consider the space of all degree-two polynomials---note that these are parameterized by a quadratic form $f(x) = x^{\dagger} A x$, where $A \in \mathbb{C}^{n \times n}$. Crucially, depending on the choice of the coefficients $A$, this polynomial will be invariant to a different group action. One well-known quadratic invariant is the \textit{power spectrum},
% One classic method for constructing a translation-invariant map is to compute the \textit{power spectrum}, 
in which the signal is transformed into the frequency domain via projections onto a basis of complex functions $\rho_i(x) = e^{i \omega_i x}$. The transform is computed using matrix multiplications by using the DFT matrix $z = Wx$., where each row $w_i$ is a discretely sampled basis function. The power of a given frequency is computed by $P_{w_i}(x) = z_i^* z_i$. For a given row $w$, we see 
\begin{align}
    P_{w}(x) &= (w^T x)^* (w^T x)\\
    &= (w_1 x_1 + w_2 x_2  + ... + w_N x_N)^* (w_1 x_1 + w_2 x_2  + ... + w_N x_N)\\
    &= \sum_{i,j} w_i^* w_j x_i^* x_j\\
    &= x^{\dagger} A x, \text{where $A = w_i^* w_j$}
\end{align}


% aim to find a function that maps signals related by group transformations to the same point. The symmetric polynomials, being invariant to permutations, may seem like a natural choice for this purpose. However, they lack selectivity and can map different transformed signals to the same point.

% To address this limitation, we turn our attention to the power spectrum, which guarantees that signals with equivalent power values are mapped to the same point. Upon closer examination, we discover that the power spectrum can be expressed as a quadratic polynomial, revealing a fascinating connection between invariant polynomials and symmetric matrices. By appropriately choosing the coefficients of the polynomial, we can construct polynomials that are invariant to different group actions, thereby capturing the desired invariance properties.

\textit{The connection between this polynomial ansatz, learning, and recovering group structure}
The central challenge in learning invariant mappings lies in parameterizing the space of invariant functions in a form amenable to gradient methods. Notably, the choice of weights or coefficients in the polynomial corresponds to the group structure we aim to learn. Consequently, by learning the weights that yield an invariant polynomial, we can effectively extract information about the underlying group from data.
% We seek to determine the functional form that encompasses the desired invariances, enabling us to learn an invariant polynomial solely from data.


\textit{The problem of uniqueness.}

However, a key question arises: Are the weights uniquely determined to achieve the desired invariances? Our research provides an affirmative answer to this question. We demonstrate that the solutions, which capture group structure and yield invariant polynomials, are unique not only for second-order polynomials but for polynomials of any degree, allowing us to express increasingly complex invariances. This remarkable theorem establishes a profound connection between invariant polynomials and the irreducible representations of the group.

The implications of this finding are profound. It not only enables us to formulate the problem of learning invariant polynomials and extract group structure but also suggests that the degree-2 case can be leveraged to construct solutions for higher-degree polynomials, leading to enhanced completeness properties. In our paper, we provide a detailed exposition of the subject, including background information on groups and group representations. We present the groundbreaking theorem, showcasing the uniqueness of the solutions for both commutative and non-commutative groups—a result never before achieved. Additionally, we demonstrate the practical utility of this theorem by constructing power spectral networks, which exhibit desirable theoretical guarantees for invariance and the ability to learn group structure from data. Furthermore, we highlight the simplicity and computational efficiency of this novel architecture, offering tangible benefits in training and computation.

\textit{Backing out of the intro, our contributions, describing the structure of the paper}
In summary, the findings presented in this paper shed light on the intricate relationship between invariant theory and machine learning. By leveraging the principles of invariant theory, we can uncover the underlying structure of groups and devise invariant mappings that facilitate robust learning from data. Our work not only establishes the uniqueness of solutions for constructing invariant polynomials but also introduces a new architecture, based on power spectral networks, that exhibits superior computational efficiency and theoretical guarantees.

The remainder of this paper is organized as follows. In Section 2, we provide a comprehensive background on groups and their representations, laying the foundation for our subsequent analysis. We delve into the key concepts and mathematical tools necessary for understanding the intricacies of invariant theory in the context of machine learning.

Section 3 constitutes the crux of our research, where we present the main theorem that establishes the uniqueness of solutions for constructing invariant polynomials for both commutative and non-commutative groups. 
% This result sheds light on the fundamental nature of invariant polynomials and their connection to the irreducible representations of groups.

In Section 4, we demonstrate the practical implications of our findings by introducing power spectral networks—a novel architecture that capitalizes on the theoretical guarantees provided by the invariant polynomials. We showcase the computational simplicity and efficiency of this architecture, illustrating its superior performance in learning and capturing group structure from data. Additionally, we discuss the advantages of leveraging the degree-2 case to construct solutions for higher-degree polynomials, further enhancing the completeness properties of the learned invariance, in particular, in the construction of complete invariants using the bispectrum.

% Finally, in Section 5, we conclude our paper by summarizing the main contributions of our work and highlighting its significance in the field of machine learning and invariant theory. We discuss potential future directions for research and applications of our findings in various domains, emphasizing the wide-ranging impact that understanding and utilizing invariant mappings can have on the development of robust and interpretable machine learning algorithms.

% In summary, this paper provides a comprehensive exploration of invariant theory from a machine learning perspective. By bridging the gap between these two domains, we uncover the deep connections between group structures and invariant mappings, enabling the construction of powerful and reliable machine learning models. Our research not only advances the theoretical understanding of invariant theory but also offers practical insights and methodologies that can revolutionize the way we learn from data.


